Measurement-based Admission Control in Sliced Networks: A Best Arm Identification Approach

In sliced networks, the shared tenancy of slices requires adaptive admission control of data flows, based on measurements of network resources. In this paper, we investigate the design of measurement-based admission control schemes, deciding whether a new data flow can be admitted and in this case, on which slice. The objective is to devise a joint measurement and decision strategy that returns a correct decision (e.g., the least loaded slice) with a certain level of confidence while minimizing the measurement cost (the number of measurements made before committing to the decision). We study the design of such strategies for several natural admission criteria specifying what a correct decision is. For each of these criteria, using tools from best arm identification in bandits, we first derive an explicit information-theoretical lower bound on the cost of any algorithm returning the correct decision with fixed confidence. We then devise a joint measurement and decision strategy achieving this theoretical limit. We compare empirically the measurement costs of these strategies, and compare them both to the lower bounds as well as a naive measurement scheme. We find that our algorithm significantly outperforms the naive scheme (by a factor $2-8$).

==> Sections/4.AnythingGoes.tex <==
\section{Identifying any Available Slice}\label{sec:anythinggoes}

With this first admission criterion, we wish to identify {\it any} available slice using a minimum number of measurements. This problem resembles the thresholding bandit problem \cite{locatelli2016}. In the latter, the decision maker needs to identify the set of {\it all} slices below the threshold, which is arguably easier since there is in this case a unique correct answer, see \cite{degenne2019pure} and \cite{garivier2021nonasymptotic} for a discussion. Our problem is also close to those addressed in  \cite{kaufmann2018sequential}, where the goal is to identify whether there exists a slice below the threshold (here, we wish to identify one such slice if any). 

%In the first approach, the agent is asked to first identify if any arm $k$ is available (has a load $\mu_k$ smaller than $\gamma$) and if so, to name \emph{one} available arm  without regard to order. Defining $k_\star$ to be the arm with lowest mean and $\mu_\star = \mu_{k_\star}$, on this problem, then, 
%%
%$$C(\mu) = \begin{cases}
%	\{k: \mu_k < \gamma\} & \text{if } \mu_\star < \gamma \\
%	\{Reject\} & \text{otherwise.}
%\end{cases} $$
% Maybe reference to SEQ lowest mean testing is unnecessary here? We are using Any Low Arm from Degenne et al anyway

%We define $d(\mu_1, \mu_2)$ to be the KL-divergence between two members of the same exponential family with means $\mu_1$ and $\mu_2$, respectively, and in particular $d_B(p, q)$ to be this KL-divergence when $p$ and $q$ are means of Bernoulli distributions. We define $k_\star$ to be the arm with lowest mean and $\mu_\star = \mu_{k_\star}$. Algorithms consist of a sampling rule $\{k_t(\mathcal{F}_{t-1})\}_{t=1}^\infty$ (where $\mathcal{F}_t$ is the filtration generated by events up to and including time $t$), a terminal decision rule $D$, and a stopping time $\tau_\delta$. We say that an algorithm is $\delta$-correct on $\mathcal{M}$ if, for all  $\nu \in \mathcal{M}$, a) the algorithm stops in finite time almost surely and b) outputs a correct answer to the question above with probability at least $1-\delta$

\subsection{Lower bound on the average measurement cost}

To identify a fundamental cost limit satisfied by any $\delta$-PC algorithm, one can leverage the classical change-of-measure arguments first introduced by \cite{lai1985} to derive regret lower bound in stochastic bandits, and then adapted in \cite{garivier2016optimal} to pure exploration problems in bandits. However, as recently discussed in \cite{degenne2019pure} and \cite{garivier2021nonasymptotic}, deriving sample complexity lower bounds is here complicated by the fact that there are multiple correct answers. 

We introduce the following notations. Let $\Lambda$ be the $(K-1)$-dimensional simplex $\Lambda=\{ w\in [0,1]^K: \sum_kw_k=1\}$. We denote by $d(\mu, \nu)$ the Kullback-Leibler divergence (KL-divergence) between two distributions parametrized by $\mu$ and $\nu$, respectively.  $d_B(\mu, \nu)$ denotes this KL-divergence in the case of Bernoulli distributions. In the sequel, to avoid pathological cases where one cannot identify an available slice even with an infinite number of measurements, we assume that $\mu_\star \neq \gamma$. The following result is a corollary of Theorem 1 in \cite{degenne2019pure} and provides a sample complexity lower bound for any of the three admission criteria. 

\begin{proposition} For any admission criteria, the sample complexity of any $\delta$-PC algorithm satisfies, for any $\mu$ such that $\mu_\star \neq \gamma$, $\mathbb{E}_\mu[\tau] \geq T(\mu)d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
		T(\mu)^{-1} =\max_{k \in {\cal C}(\mu)} \max_{{w} \in \Lambda} \inf_{\lambda: k \notin {\cal C}(\lambda)} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell}).
	\end{equation}
	\label{prop:GeneralLowerBound}
	\end{proposition}
	%

The above lower bound, defined by the {\it characteristic} time $T(\mu)$, is not explicit, and in general hard to compute. We may interpret this lower bound as follows. Let ${\cal  C}^\star(\mu)\subseteq {\cal C}(\mu)$ the set of maximizers over $k$ of $F(\mu,k)=\max_{{w} \in \Lambda} \inf_{\lambda: k \notin {\cal C}(\lambda)} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell})$. Slices in ${\cal  C}^\star(\mu)$ are the {\it easiest} correct answers to identify, and an optimal algorithm should sample as to output one of these slices. Identifying $k\in {\cal  C}^\star(\mu)$ is done with minimal sample complexity when the sampling rule realizes the allocation of slice draws defined by ${w}^\star(\mu, k) = \arg\max_{{w} \in \Lambda}F(\mu,w,k)$. The following proposition provides an explicit expression of the lower bound for the any-available-slice identification problem. 

\begin{proposition}
For the any-available-slice problem, we have, for any $k\in {\cal C}(\mu)$ and all $\ell\in [K]$,
\begin{equation}
w_\ell^\star(\mu, k) = \mathds{1}_{(k = 0)}\frac{d(\mu_\ell, \gamma)^{-1}}{\sum_{j=1}^{K}d(\mu_j, \gamma)^{-1}} + \mathds{1}_{(k=\ell)}.
	\label{eq:OptimalAnythingProportions}
	\end{equation}
%\begin{equation}
%w_k^\star(\mu, \ell) = \begin{cases}
%			\frac{(d(\mu_\ell, \gamma))^{-1}}{\sum_{j=1}^{K}(d(\mu_j, \gamma))^{-1}} & \text{if } k= 0 \ \ \text{(reject)},\\
%	\mathds{1}(\ell = k) & \text{otherwise.}
%\end{cases}
%	\label{eq:OptimalAnythingProportions}
%	\end{equation}
%	%
In particular, the sample complexity of any $\delta$-PC algorithm satisfies $\mathbb{E}_\mu[\tau] \geq T_1(\mu)d_B(\delta,1-\delta)$		
where
	%
	\begin{equation}
		T_1(\mu) = \begin{cases}
			d(\mu_\star, \gamma)^{-1} & \text{if } \mu_\star < \gamma, \\
			\sum_{j=1}^K d(\mu_j, \gamma)^{-1} & \text{otherwise.}
		\end{cases}
	\end{equation}
	\label{prop:AnythingLowerBound}
\end{proposition}

The proof of the above Proposition and those of the other results presented in this paper are postponed to the appendix. Note that in the any-available-slice problem, the easiest slices to identify are those with minimum load: 
\begin{equation}\label{eq:easy1}
{\cal C}^\star(\mu)=\left\{
\begin{array}{ll}
\{k: \mu_k=\mu_\star\} & \hbox{ if } \mu_\star<\gamma,\\
\{0\}& \hbox{ otherwise.}
\end{array}
\right.
\end{equation}
Further note that the optimal sampling rule suggested by the lower bound is {\it discountinuous}: if $\mu_\star < \gamma$,  it samples only slices with load $\mu_\star$, but if $\mu_\star > \gamma$ it samples all slices with different frequencies.

%\begin{proof}[Proof sketch] 
%	The proof logic closely follows that of \cite{kaufmann2018sequential}. If $\mu_\star > \gamma$, the agent needs to, individually, sample all arms and verify that their mean is greater than $\gamma$. If, on the other hand, $\mu_\star < \gamma$, it suffices to verify that any particular arm has mean smaller than $\gamma$. The most efficient way, for an oracle, to accomplish this is to sample only $k_\star$. With these facts in mind, the proposition follows from the fundamental lemma in \cite{garivier2019explore}. The full proof can be found in Appendix \ref{appx:LowerBoundProofs}.
%\end{proof}






\subsection{Track-and-Stop algorithm}
%% TODO: Decide whether to keep Multiple correct answers framework, and if so, describe it, or to rewrite with different framework.

Next, we describe the Track-and-Stop (\textsc{TaS}) algorithm, a generic algorithm that will be instantiated for the three identification problem, and establish its asymptotic optimality (when $\delta$ approaches 0) for the any-available-slice problem.

\medskip
\noindent
{\it Sampling rule.} The sample complexity lower bound and its interpretation provide the design principle of the sampling rule. In this paper, we follow the Track-and-Stop framework developed in \cite{garivier2016optimal} for best arm identification problem in bandits. In this framework, extended to our problem, the $t$-th measured slice is chosen as follows. $\mu$ is estimated by its sample mean $\hat{\mu}(t-1)$ from the $(t-1)$-th first measurements. $\hat{\mu}(t-1)$ then replaces $\mu$ in $w^\star({\mu},k)$ and ${\cal C}^\star(\mu)$, i.e., these are approximated by $\hat{w}^\star(t,k):=w^\star(\hat{\mu}(t-1),k)$ and $\hat{\cal C}(t):={\cal C}^\star(\hat{\mu}(t))$, respectively. Finally, we select a target slice\footnote{The subscript 'E' stands for 'Easiest'.} $k_E(t)$ from $\hat{\cal C}^\star(t)$, and sample the slice $k_t$ to measure using the proportions $\hat{w}^\star(t,k_E(t))$. The way $k_E(t)$ is selected from $\hat{\cal C}^\star(t)$ matters in general, and here, we always select the slice with minimal index. The algorithm described above works as long as we can make sure that $\hat{\mu}(t)$ converges to $\mu$ a.s.. To this aim, the sampling rule includes a {\it forced exploration} phase: after $t$ measurements, slices that have not been measured more than $\sqrt{t}$ times are measured. If the algorithm is not in a forced exploration phase, it tracks the allocation $\hat{w}^\star(t,k_E(t))$, i.e., it measures the slice $k_t\in \arg\max_k t\hat{w}^\star_k(t,k_E(t))-N_k(t-1)$, where $N_k(t-1)$ is the number of times $k$ has been measured so far. Finally note that the sampling rule depends on the functions $\mu\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$. For the any-available-slice problem, these are given by (\ref{eq:OptimalAnythingProportions}) and (\ref{eq:easy1}), respectively.

\medskip
\noindent
{\it Stopping rule.} The stopping rule we use is classical and relies on a similar stopping criterion as in all previously devised pure exploration algorithms. Specifically, it is based on the Generalized Likelihood Ratio (GLR) statistics $Z_{k,k'}(t)$ evaluating the probabilities that given the observations, the targeted correct answer is $k=k_E(t)$ or $k'$, see details in \cite{garivier2016optimal} and \cite{degenne2019pure}. We stop when these GLR are large enough. The resulting statistical test can summarized by comparing $\inf_{\lambda: \hat{k}(t) \notin \mathcal{C}(\lambda)} \sum_{k=1}^K N_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$ to an exploration threshold $f_\delta(t)$ appropriately chosen.  

\medskip
\noindent
{\it Decision rule.} When the algorithm stops measuring after $\tau$ measurements, it returns the slice $k_E(\tau)$. The pseudo-code of the algorithm is presented in Algorithm \ref{alg:TaS}. There, $N(t)$ denotes the vector counting the number of times each slice has been measured up to time $t$ (such that $\sum_{k=1}^K N_{k}(t) = t$). 

%To utilize the lower bounds in practice, we will employ versions of ``Track-and-Stop'' with D-tracking \cite{garivier2016optimal}, so named for the use of a \emph{tracking} sample rule. Let $\hat{\mu}(t)$ be the sample mean of each arm at time $t$ and let $N(t)$ be the vector counting the number of times each arm has been pulled up to time $t$ (such that $\sum_{k=1}^K N_{k}(t) = t$). We will assume that we have access to an oracle $\hat{w}^\star(\mu)$ which for any answer $\ell \in \mathcal{C}(\hat{\mu}(t))$ and any given time $t$ can calculate the optimal proportions as $\hat{w}(t) = \hat{w}^\star(\hat{\mu}(t), \ell)$. Such an oracle will generally employ lower bound results such as that in \ref{prop:AnythingLowerBound}. Further, we denote by $\hat{k}(t)$ the algorithm's output at time $t$, which will be generated by a \emph{best arm rule} $\hat{k}^\star(\mu)$. Let $f_\delta(t)$ be a stopping function. We describe the algorithm as presented by \cite{degenne2019pure} in Algorithm \ref{alg:TaS}.

\begin{algorithm}[t]
	\caption{Track-and-Stop (\textsc{TaS})}
	\label{alg:TaS}
	\begin{algorithmic}

		% I don't like the notation for the empirical best arm rule... Is there anything better?		
		%\Require Best arm rule $\hat{k}^\star: \mathcal{M} \to [K]$
		%\Require Oracle weight function $\hat{w}^\star:\mathcal{M} \times [K] \to \Lambda$
		%Oracle functions $w^\star(\mu,k)$ and ${\cal C}^\star(\mu)$
		\State {\bf Input:} Oracle functions $(\mu,k)\mapsto w^\star(\mu,k)$ and $\mu\mapsto {\cal C}^\star(\mu)$
		\State {\bf Initialization:} $\hat{\mu}(0) = 0$, $N(0) = 0$
		\For{$t=1,...$}
		\State ${k}_E(t)\leftarrow  \min {\cal C}^\star(\hat{\mu}(t-1))$
		\State $Q(t)\leftarrow \inf_{\lambda: {k}_E(t) \notin \mathcal{C}(\lambda)} \sum_{k=1}^K N_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$
		\If{$Q(t) > f_\delta(t)$}
		\State Stop and return ${k}_E(t)$
		\EndIf
		\State $\hat{w}(t)\leftarrow  {w}^\star(\hat{\mu}(t-1), {k}_E(t))$
		\If{$\exists k: N_{k}(t-1) < \sqrt{t}$}
		\State $k_t \leftarrow \arg\min_k N_{k}(t-1)$
		\Else
		\State $k_t \leftarrow \arg \max_k t \hat{w}_{k}(t) - N_{k}(t-1)$
		\EndIf
		\State Measure slice $k_t$ and observe $X_{k_t}(t)$
		\State  $N(t) \leftarrow N(t-1) + {\bf e}_{k_t}$
		\State $\hat{\mu}(t)\leftarrow \hat{\mu}(t-1) + \frac{1}{N_{k_t}(t)}(X_{k_t}(t) - \hat{\mu}_{k_t}(t-1)) {\bf e}_{k_t}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

%The idea behind Algorithm \ref{alg:TaS} is to \emph{track} the empirical weights $\hat{w}(t)$ and sample as if they were the true oracle weights, stopping when the probability of making an error is sufficiently small. It is applicable on many problems in its current form, but needs explicit methods to calculate $\hat{k}^\star$ and $\hat{w}^\star$ before implementation.
%For the problem of identifying any available slice, we select $\hat{k}^\star(\mu) = k_\star \mathds{1}_{(\mu_\star < \gamma)} $. Further, for the weight function $\hat{w}^\star$ we use $w^\star$ as defined in equation \eqref{eq:OptimalAnythingProportions}. 

\medskip
The following theorem, proved leveraging results from \cite{degenne2019pure}, establishes the asymptotic (as $\delta$ goes to 0) optimality of \textsc{TaS} for the any-available-slice problem, up to a factor 2. 

\begin{theorem}
Let \textsc{TaS} be instantiated for the any-available-slice problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalAnythingProportions}) and (\ref{eq:easy1}), respectively. Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k_\star$ is unique,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\mathbb{E}_\mu[\tau]}{d_B(\delta,1-\delta)} \leq 2T_1(\mu).
	\end{equation}
	\label{the:AlgResults}
\end{theorem}

We conclude this section by remarking that for $\mu$ such that $k_\star$ is not unique, we would need to add a component to the algorithm to avoid the oscillation of $k_E(t)$ between these slices with minimal load. This is done in \cite{degenne2019pure} by introducing a {\it sticky} component to the algorithm. We could follow this idea, but for simplicity and clarity of the paper, prefer to restrict our attention to the cases where $k_\star$ is unique. 



%This is a direct consequence of Theorem 11 in \cite{degenne2019pure} since the \emph{Any available slice} problem is equivalent to the \emph{Any Low Arm} problem in the framework of that paper. Notably, since we by previous measurement cost bounds showed that
%%
%$$\liminf_{\delta \to 0} \frac{\E{\tau_\delta}}{\log(1/\delta)} \geq T_1(\mu)$$
%%
%for any $\delta$-correct algorithm, this implies that \textsc{TaS} is asymptotically optimal. This does not translate to optimality in moderate confidence regions, but it does give some confidence in this choice of algorithm when the confidence level is high.




==> Sections/5.Packing.tex <==
\section{Identifying the Packing Slice}\label{sec:packing}

For the second admission criterion, the objective is to identify $k^\star$, the packing slice (if it exists). Recall that if $\mu_\star<\gamma$, $k^\star=\arg\max_{k:\mu_k< \gamma} \mu_k$. For simplicity, we will restrict our attention to slice loads $\mu$ such that the packing slice is unique when it exists. The identification problem slightly resembles the dose ranging problem addressed for Gaussian arms in \cite{garivier2018thresholding}, but there, the objective is to find the arm with the reward the closest to a given threshold -- not necessarily below, as in our case.   



%In the second approach, the agent is asked to identify the (assumed to be unique) \emph{packing} arm $k^\star$ with the greatest mean $\mu^\star < \gamma$, so that for all arms $k\neq k^\star$, either $\mu_k < \mu^\star$ or $\mu_k > \gamma$. This is useful for admission control since it allows us to ``pack'' services into slices, potentially leaving room for future demanding services.

\subsection{Lower bound on the average measurement cost}

As for the any-available-slice problem, we can derive lower bounds on the average measurement cost satisfied by any $\delta$-PC algorithm. To state these bounds, we distinguish two cases: (i) when $\mu_\star<\mu^\star<\gamma$ (which means that there exists a packing slice and that it is different from the slice with minimum load); and (ii) when either $\mu_\star > \gamma$ (the correct answer is 0) or $\mu_\star=\mu^\star<\gamma$ (there is a unique available slice). 

For the first case only, we introduce the following notations. For any $\mu, \nu$, $\alpha\in [0,1]$, let $I_\alpha(\mu, \nu) = \alpha d(\mu, \alpha \mu + (1-\alpha)\nu) + (1-\alpha) d(\nu, \alpha \mu + (1-\alpha)\nu)$ be a weighted symmetrization of the KL divergence with weight $\alpha$. Define the information function of slice $k$ in relation to slice $k^\star$ as $g_k(x) = (1+x)I_{\frac{1}{1+x}}(\mu^\star, \mu_k)$. Further, let $x_k^\star(y) = g_k^{-1}(y)$, and $x_{k^\star}^\star(y)=1$ for all $y$ by convention. Let $\mu_k'(y) = \frac{\mu^\star + \mu_a x_k^\star(y)}{1 + x_k^\star(y)}$, and finally define the function $F_P$ by
\begin{equation}
		F_P(y)= \sum_{k:\mu_k< \mu^\star} \frac{d(\mu^\star, \mu_k'(y))}{d(\mu_k, \mu_k'(y))}.
	\end{equation} 
The next proposition provides an explicit expression of the sample complexity lower bound for the problem of identifying the packing slice. Its proof starts from the results of Proposition \ref{prop:GeneralLowerBound}, and can be found in appendix. 

\begin{proposition}
Consider a $\delta$-PC algorithm with sample complexity $\tau$.\\
(i) Assume that $\mu$ satisfies $\mu_\star < \mu^\star < \gamma$. Let $z^\star = \min(d(\mu^\star, \gamma), y^\star)$ where $y^\star$ is the unique solution to the equation $F_P(y) = 1$ ($y^\star$ and $z^\star$ are well defined). Then, $\E[\mu]{\tau} \geq T_2(\mu)d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
		T_2(\mu) = \sum_{k: \mu_k > \mu^\star} d(\mu_k, \gamma)^{-1} +
		\frac{1}{z^\star}\sum_{k:\mu_k<\gamma} x_k^\star(z^\star).
	\end{equation}
	%
	Furthermore, we have, for any $k \in [K]$,
	%
	\begin{equation}
		w_k^\star(\mu, k^\star) =\frac{1}{T_2(\mu)} \left( \frac{x_k^\star(z^\star)\mathds{1}_{(\mu_k < \gamma)}}{z^\star} + \frac{\mathds{1}_{(\mu_k > \gamma)}}{d(\mu_k, \gamma)} \right).
		% \begin{cases}
		%	\frac{x_a(z^\star)}{z^\star T_2(\mu)}	&	\text{if } \mu_k < \mu^\star \\
		%	\frac{1}{z^\star T_2(\mu)} 			&	\text{if } k = k^\star \\
		%	\frac{1}{d(\mu_k, \gamma)T_2(\mu)}	&	\text{otherwise.}
		%\end{cases}
		\label{eq:OptimalPackingProportions}
	\end{equation}
	%
(ii) Assume that $\mu$ satisfies $\mu_\star > \gamma$ or $\mu_\star = \mu^\star < \gamma$. Then, $\E[\mu]{\tau} \geq T_2(\mu)d_B(\delta,1-\delta)$ where
	%
	\begin{equation}
		T_2(\mu) = \sum_{k=1}^K d(\mu_k, \gamma)^{-1}.
	\end{equation}
	%
	Furthermore, we have, for any $k \in [K]$ and any $\ell \in \mathcal{C}(\mu)$ (so $\ell = 0$ if $\mu_\star > \gamma$ and $\ell = k^\star$ if $\mu_\star = \mu^\star$), 	%
	\begin{equation}
		w_k^\star(\mu, \ell) =\frac{d(\mu_k,\gamma)^{-1}}{T_2(\mu)}.
		% \begin{cases}
		%	\frac{x_a(z^\star)}{z^\star T_2(\mu)}	&	\text{if } \mu_k < \mu^\star \\
		%	\frac{1}{z^\star T_2(\mu)} 			&	\text{if } k = k^\star \\
		%	\frac{1}{d(\mu_k, \gamma)T_2(\mu)}	&	\text{otherwise.}
		%\end{cases}
		\label{eq:OptimalPackingProportionsDegenCase}
	\end{equation}
\label{prop:PackingLowerBound}
\end{proposition}


%\begin{proof}[Proof sketch]
%	The full proof can be found in Appendix \ref{appx:LowerBoundProofs}. In general, there are three ways to create an alternate problem $\lambda$ where $k^\star$ is no longer optimal
%	
%	\begin{enumerate}
%		\item For some arm $k$ with $\mu_k > \gamma$, modify this arm such that $\lambda_k < \gamma$.
%		\item For some arm $k$ with $\mu_k < \mu^\star$, modify this arm and $k^\star$ such that $\lambda_k > \lambda_{k^\star}$. 
%		\item Modify $k^\star$ such that $\lambda_{k^\star} > \gamma$.
%	\end{enumerate}
%	
%	First, we note that arms such that $\mu_k > \gamma$ are only treated in condition 1. Further, there is no need to compare them to $k^\star$ directly, since any perturbation that makes $\lambda_k < \gamma$ suffices to confuse the agent. Thus, the agent needs to verify that all these arms are greater than $\gamma$, which from the thresholding means problem we know requires to pull arm $k$ at least $d_B(\delta,1-\delta)/d(\mu_k,\gamma)$ times. This leads to the first summand in $T_2$, and we will not need to consider these arms any more. 
%	
%	Similarly, the third condition tells us that arm $k^\star$ must be pulled at least $d_B(\delta,1-\delta)/d(\mu^\star,\gamma)$ times. The second condition adds a wrinkle to this, however. The second condition can be seen as solving a best arm identification problem for all arms $k$ with $\mu_k < \gamma$. From \cite{garivier2016optimal}, we know that this implies that for all arms, they need to be pulled $n_k$ times and further, for symmetry reasons, the quantity $g_k(n_k/n_{k^\star})$ is identical for all arms $k \neq k^\star$. Furthermore, we also know that, in the unconstrained case, this quantity is identical to $y^\star$ as given in the proposition. It can be shown that if $y^\star \leq d(\mu^\star,\gamma)$, the arm $k^\star$ will be sufficiently pulled by a best arm identification algorithm and so, we have the second case in the second term of $T_2$. However, if this is not the case we still find that the quantities $g_k(n_k/n_{k^\star})$ are equal but that they are also equal to $d(\mu^\star, \gamma)$. This leads to the first case.
%	
%	
%\end{proof}

Remember that we made the assumption that $k^\star$ is unique when it exists. When this is not the case, the lower bound of Proposition \ref{prop:PackingLowerBound} would suggest an infinite sample complexity. We can circumvent this difficulty by accepting \emph{overlapping hypotheses} \cite{garivier2021nonasymptotic}, i.e., we can require the algorithm to output a slice $k$ with mean $\mu^\star - \varepsilon \leq \mu_k \leq \mu^\star$ with probability $1 - \delta$ for some tolerance threshold $\varepsilon > 0$. For clarity of the exposition, we omit the rather lengthy theoretical analysis required to bound the sample complexity of such algorithms.


\subsection{Track-and-Stop algorithm}
Under the assumption of a unique packing arm $k^\star$, we can use \textsc{TaS} (Algorithm \ref{alg:TaS}) to solve the packing-slice identification problem. To this aim, we instantiate the algorithm using: 
\begin{equation}\label{eq:css}
{\cal C}^\star(\mu) = \left\{
\begin{array}{ll}
\{ k^\star\} &\hbox{ if }\mu_\star<\gamma,\\
\{0\}&\hbox{ otherwise,}
\end{array}
\right.
\end{equation}
 and the weight function $w^\star$ defined in  (\ref{eq:OptimalPackingProportions}) and (\ref{eq:OptimalPackingProportionsDegenCase}) depending on the case.

\begin{theorem}
Let \textsc{TaS} be instantiated for the packing-slice identification problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalPackingProportions}),  (\ref{eq:OptimalPackingProportionsDegenCase}) and (\ref{eq:css}). Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k^\star$ is unique when it exists,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\E[\mu]{\tau}}{d_B(\delta,1-\delta)} \leq 2T_2(\mu).
	\end{equation}
	\label{the:PackingAlg}
\end{theorem}


==> Sections/6.MinimumLoad.tex <==
\section{Identifying the Least Loaded Available Slice}\label{sec:minimumload}

For the last admission criterion, we wish to identify the least loaded slice $k_\star$ provided it is below the threshold $\gamma$. This criterion is sometimes preferable to ensure that the load is evenly distributed between slices. The corresponding identification problem is related to the classical Best Arm Identification problem \cite{garivier2016optimal} with the important difference that here if the load of $k_\star$ is above the threshold $\gamma$, the correct decision is to reject the flow. We assume again to simplify the presentation that $k_\star$ is unique.

\subsection{Lower bound on the average measurement cost}

To state the lower bound, we distinguish two cases: (i) when $\mu_\star<\gamma$ (the correct answer is $k_\star$); (ii) when $\mu_\star>\gamma$ (the correct answer is $0$). For the first case only, we will use the following notation. Define $h_k(x):=(1+x)I_{\frac{1}{1+x}}(\mu_\star, \mu_k)$, $x_{\star, k}(y) := h_k^{-1}(y)$ (with, again, $x_{\star, k_\star}(y)= 1$ for all $y$) and $\mu_k''(y) := \frac{\mu_\star + \mu_k x_{\star, k}(y)}{1 + x_{\star, k}(y)}$  and finally $F_{ML}$ is the function
%
\begin{equation}
	F_{ML}(y)= \sum_{k:\mu_k> \mu_\star} \frac{d(\mu_\star, \mu_k''(y))}{d(\mu_k, \mu_k''(y))}.
\end{equation}  
$F_{ML}$ is defined whenever there exist at least two arms (in any other case, the problem is trivial) and is monotonic.

\begin{proposition}		
Consider a $\delta$-PC algorithm with sample complexity $\tau$.\\
(i) Assume that $\mu$ satisfies $\mu_\star < \gamma$. Let $z_\star = \min(d(\mu_\star, \gamma), y_\star)$ where $y_\star$ is the unique solution to the equation $F_{ML}(y) = 1$ ($y_\star$ and $z_\star$ are well defined). Then we have $\E[\mu]{\tau} \geq T_3(\mu)d_B(\delta,1-\delta)$ where 
	\begin{equation}
		T_3(\mu) = \frac{1}{z_\star} \sum_{k = 1}^K x_{\star, k}(z_\star).
	\end{equation}
	%
	Furthermore, we have, for all $k \in [K]$,
	%
	\begin{equation}
		w_k^\star(\mu ,k_\star) = \frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}.
		%\begin{cases}
		%	\frac{1}{z_\star T_3(\mu)} &	\text{if } k=k_\star \\
		%	\frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}		& \text{otherwise.}
		%\end{cases}
	\label{eq:OptimalMinimumProportions}
	\end{equation}
(ii) Assume that $\mu$ satisfies $\mu_\star > \gamma$. Then, we have $\E[\mu]{\tau} \geq T_3(\mu)d_B(\delta,1-\delta)$ where 
	\begin{equation}
		T_3(\mu) = \sum_{k = 1}^K d(\mu_k, \gamma)^{-1}.
	\end{equation}
	%
	Furthermore,  we have, for all $k \in [K]$,	%
	\begin{equation}
		w_k^\star(\mu,0) = \frac{d(\mu_k, \gamma)^{-1}}{T_3(\mu)}. 
		%\begin{cases}
		%	\frac{1}{z_\star T_3(\mu)} &	\text{if } k=k_\star \\
		%	\frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}		& \text{otherwise.}
		%\end{cases}
		\label{eq:OptimalMinimumProportionsDegenCase}
	\end{equation}
	\label{prop:MinimumLowerBound}
\end{proposition}

%\begin{proof}[Proof sketch]
%	The set of confusing problems $\neg k_\star$ can be written as the union of $\Lambda_2 = \{\lambda \in \mathcal{M}: \exists a \neq _\star: \lambda_a < \lambda_{k_\star} \}$ and $\Lambda_3 = \{\lambda \in \mathcal{M}: \lambda_{k_\star} > \gamma \}$. The rest of the analysis is completely analogous to the one concerning $\Lambda_2$ and $\Lambda_3$ in the proof of Proposition \ref{prop:PackingLowerBound} (see Appendix \ref{appx:LowerBoundProofs}).
%\end{proof}

The expressions of the sample complexity lower bounds in the packing-slice and least-slice identification problems enjoy a similar form. However, they are quantitatively often very different. Indeed, $\mu^\star$ is often much closer to $\gamma$ than $\mu_\star$, and as a result, $d(\mu^\star, \gamma) \ll d(\mu_\star, \gamma)$ and identifying the packing-slice requires much more measurements. 

\subsection{Track-and-Stop algorithm}

Under the assumption of a unique least loaded slice $k_\star$, we can use \textsc{TaS} (Algorithm \ref{alg:TaS}) to solve the least-loaded-slice identification problem. To this aim, we instantiate the algorithm using: 
\begin{equation}\label{eq:css2}
{\cal C}^\star(\mu) = \left\{
\begin{array}{ll}
\{ k_\star\} &\hbox{ if }\mu_\star<\gamma,\\
\{0\}&\hbox{ otherwise,}
\end{array}
\right.
\end{equation}
 and the weight function $w^\star$ defined in  (\ref{eq:OptimalMinimumProportions}) and (\ref{eq:OptimalMinimumProportionsDegenCase}) depending on the case.

\begin{theorem}
Let \textsc{TaS} be instantiated for the least-loaded-slice identification problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalMinimumProportions}),  (\ref{eq:OptimalMinimumProportionsDegenCase}) and (\ref{eq:css2}). Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k_\star$ is unique,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\E[\mu]{\tau}}{d_B(\delta,1-\delta)} \leq 2T_3(\mu).
	\end{equation}
	\label{the:MinimumAlg}
\end{theorem}



==> Sections/FutureWork.tex <==
Mean rewards of arms evolve as a stochastic process with 'memory'. 
$\Rightarrow$ Sequential best arm identification in non-stationary environments


==> Tech report version/Sections/1.Introduction.tex <==
\section{Introduction}\label{sec:intro}

In next generation telecom networks, the network resources will be divided and allocated to multiple slices shared between several slice tenants \cite{9295415}. With limited to no knowledge of the behavior of other tenants, a slice tenant must, in order to uphold certain service guarantees, decide to accept or reject incoming data flows, while adapting to rapidly changing network occupancy levels. This is further complicated by an unclear dependency of the slice occupancy on the resources of individual slice components. The admission control agent must therefore measure the network resources and current utilization before an admission decision can be made, reintroducing a need for \emph{measurement-based admission control} (MBAC), a popular method in the context of call admission control which has recently fallen out of favor \cite{jamin1997measurement, gibbens1997measurement, 779194}. MBAC schemes have the advantage to adapt to uncertainties arising due to the difficulty of characterizing traffic sources or to that of estimating the available resources (in wireless networks, these evolve depending on e.g. user mobility, fading, interference). However, MBAC comes with an inherent cost since a fraction of the resources is used for the measurements. This cost can become substantial as the admission criteria grows in complexity \cite{tahaei2018cost}, especially in system with inherently scarce resources such as wireless systems \cite{camp2008measurement}. 

% Before accepting or rejecting a new data flow, Admission Control (AC) mechanisms check whether the resources available on a relevant network path are sufficient to guarantee some level of quality of service to all flows that link or server handles, should the new flow be accepted. Traditionally, AC decisions have been made either based on a-priori static traffic descriptors of data flows (which often leads to poor resource utilization \cite{brewer2010comparison}) or based on measurements \cite{jamin1997measurement, gibbens1997measurement, 779194}. Measurement-based admission control (MBAC) schemes have the advantage to adapt to uncertainties arising due to the difficulty of characterizing traffic sources or to that of estimating the available resources (in wireless networks, these evolve depending on e.g. user mobility, fading, interference). However, MBAC comes with an inherent cost since a fraction of the resources is used for the measurements. This cost can become very substantial as the admission criteria grows in complexity \cite{tahaei2018cost}, especially in system with inherently scarce resources such as wireless systems \cite{camp2008measurement}. 


In this paper, we investigate the design of MBAC strategies in multi-slice networks, where the controller has to decide whether a new data flow can be admitted and if so, on which slice. The controller  has no knowledge about the slice loads, but may gather this knowledge conducting noisy and costly measurements. 
%Such scenarios naturally arise when the server resources are shared in a decentralized manner by many users handling data flows, e.g., as in multi-slice systems with multiple tenants \cite{perveen2019dynamically, ojijo2020survey}, or decentralized channel access in wireless networks \cite{maskery2009decentralized, zhao2005decentralized}. There, the network operator must decide whether a new data flow can be accepted into one of slices or servers
%\footnote{Throughout the paper, we use the term {\it slice} to fix ideas, but it can represent any type of servers: slices, links, radio channels, etc.} 
%or must be rejected. 
To this aim, it can sequentially measure the traffic handled (over a fixed duration -- a time slot) by a selected slice, and stop whenever it believes it has gathered enough information to come up with a {\it correct} decision with some level of certainty. A correct decision should be to reject the flow if all slices are already fully loaded, or to select one of the slices that has enough available resources if any, given assumptions on the new network flow.  The objective is to devise a joint measurement and decision strategy that returns a correct decision with a certain level of confidence while minimizing the measurement cost (the number of measurements made before committing to the decision). We study the design of such strategies for several natural admission criteria specifying what a correct decision is. These criteria can consist in selecting (i) {\it any} of the slices with available resources, (ii) the most loaded slice with available resources (we refer to this slice as the {\it packing} slice), or (iii) the \emph{least loaded} slice with available resources.%\footnote{We discuss and evaluate the advantages of these criteria later in the paper.}.  

We address the design of joint measurement and decision strategies using the formalism of pure exploration in stochastic Multi-Armed Bandits (MAB). Online exploration algorithms for MAB specify an adaptive sequence of arms (for us, slices) to observe (here, the traffic handled by the selected slice in a slot), a stopping rule indicating when to output a decision, and a decision rule. For each of the aforementioned admission criteria, we first derive an explicit information-theoretical lower bound on the cost of any algorithm returning the correct decision with fixed confidence. We then devise a joint measurement and decision strategy achieving this theoretical limit. We compare empirically the costs of these strategies, and compare these cost both to the lower bound and to a naive sampling strategy. These results allow us to analyze the trade-off between measurement cost and complexity of the proposed admission criteria.


%This leads naturally to the field of \emph{Best Arm Identification with fixed confidence}, a set of adaptive sampling methods ensuring that an agent returns an in some sense \emph{correct} answer from a finite but possibly large set with a certain confidence, sampling in such a way as to minimize stopping time. In this paper, by applying such methods for each admission decision we are able to robustly guarantee minimal capacity violations and low blocking rate while maintaining minimal measurement costs, even in scenarios where no information can be saved between decisions.
%We present the following contributions.

%(i) We design a new framework for admission control with minimal measurement cost using tools from Best Arm Identification. The framework is flexible and allows for several types of admission criteria, including but not limited to (a) ``Any admissible slice'', where the agent identifies a random admissible slice while minimizing measurement cost, (b) ``Packing slice'', where the agent attempts to pack as many services into one slice as possible to enable slice vacancy and sleep time, and (c) ``Minimum load slice'', where the agent attempts to distribute the load evenly between slices to maximize Quality of Service (Section \ref{sec:models}).

%(ii) We study lower bounds on packet-level measurement cost for these three criteria and provide explicit forms for these bounds.  We then utilize existing Best Arm Identification algorithms to show how these bounds can be achieved in the context of admission control, while maintaining confidence guarantees (Sections \ref{sec:anythinggoes} - \ref{sec:minimumload}).

%(iii) Finally, we evaluate these algorithms and the different admission criteria in simulation, quantitatively showing the trade-off between admission control quality (measured with blocking probability for different service classes) and average measurement cost (Section \ref{sec:num}).






%
%However, because decisions are decentralized, tenants lack information about each other's decisions. Furthermore, varying packet rates and user mobility causes information about the current traffic to degrade over time. As such, any tenant must monitor the network resources between decision points in order to perform good admission control. 
%
%Traditionally, there have been two distinct approaches to monitoring in admission control: (i) Parameter-based approaches, which proactively reserve network resources based on statistics of peak usage, and (ii) Measurement-based approaches, which reactively gather measurements in order to make admission control decisions suited to the current network state. While parameter-based approaches are typically faster, they often lead to under-utilized networks \cite{brewer2010comparison}. In this paper, we therefore consider the latter.
%
%However, as networks grow more complicated, measurement-based approaches face new challenges. In particular, over-measuring a system can lead to degradation of performance and high energy costs. \cite{tahaei2018cost}, \cite{camp2008measurement}. Thus, new methods are needed to minimize measurement costs, both on a case-by-case basis as well as averaged over a period of time, while simultaneously maintaining high quality admission control. Furthermore, while traditional approaches such as those proposed by \cite{jamin1997measurement}, \cite{gibbens1997measurement}, \cite{779194} look at binary decisions of admitting into a single server, in modern networks it is often possible to admit incoming service requests into one of several slices, each potentially differently well equipped to accept a new service.

%Measurement-based slice admission control with measurement costs.
%
%Measurements are costly, slice load unknown. Many slices, end-to-end slices are composed by many software and hardware components that we cannot monitored. 
%
%Costs - overhead in transfer of measurement results, sampling overhead in multi-slice softwarized environment. Slices are end-to-end and may contain multiple VNFs.
%
%Guarantees on service-level performance, with a certain level of confidence. Then we solve the problem of minimizing the measurement costs subject to these guarantees. 
%
%Performance is measured by flow-level blocking rates, packet-level performance (SLA violation) and measurement cost.
%
%1. Study the flow-level performance of various Oracle-based policies.
%
%2. Learning mechanisms to implement these Oracle policies. For various policies, we get a measurements cost. And we can see the trade-of between measurement cost and flow-level blocking rates
%
%\begin{enumerate}
%	\item Packing
%	\item Trunk reservation
%	\item Random - "first discovered"
%\end{enumerate}
%
%Comparison with \cite{degenne2019pure}: they investigate a very generic pure exploration pb with multiple correct answers: lower bound and optimal algorithm. Lower bounds: not explicit and no procedure to compute them, we make the LB explicit and easy to compute.  Optimal algorithm: meta-algo requires the use some oracle that would solve the LB optimization pb. Based on explicit expression of our LB, we have simple and optimal algos. 





==> Tech report version/Sections/2.RelatedWork.tex <==
\section{Related work}

{\bf Stochastic bandit} problems have received plenty of attention since they were introduced by Thompson in the 30's and formalized by Robbins in 1952. While bandit problems were initially motivated by clinical trials, they have recently found important applications in the design of protocols and algorithms in communication networks (mostly in cognitive radio systems, see \cite{liu2010, anandkumar2011}
%, avner2019} 
and references therein, or rate adaptation in wireless systems \cite{combes2019}). Most often in bandits, the focus has been on the design of algorithms with low regret \cite{lai1985}. The problem of identifying the best arm using a minimal number of samples is more recent, see \cite{mannor2004, evendar2006} for early work. Algorithms to find the best arm with  minimal sample complexity have been developed in \cite{garivier2016optimal}. Since then, researchers have tried to extend these algorithms to more general {\it pure exploration} problems \cite{degenne2019pure}, such as \cite{garivier2018thresholding} where one searches for the arm with average reward the closest to a given threshold. In this paper, we investigate three novel pure exploration problems, each corresponding to a different admission criterion, and we use the framework developed in \cite{garivier2016optimal} to derive sample complexity lower bounds and to devise optimal algorithms based on these lower bounds. While \cite{degenne2019pure} constructed general lower bounds for such problems, they are often implicit and non-trivial to compute. Furthermore, their algorithm \emph{Sticky Track-and-Stop} cannot typically be implemented without both an explicit form of these bounds and the assumption of Gaussian random variables. By contrast, we provide explicit bounds for our admission criteria as well as an algorithm applicable for a wide class of \linebreak measurement distributions.

{\bf Admission control} methods in the context of network slicing are summarized in \cite{ojijo2020survey}. These methods vary in slice elasticity, inter vs intra-slice admission control, single vs multi-tenant systems, and use both heuristic and optimal methods. None of these methods explicitly take measurement overhead into account. As far as we are aware, this paper proposes the first approach to actually optimize the measurement strategy in admission control. It is worth noting that our admission control problems may seem similar to the problem of dynamic channel assignment in wireless networks, see e.g., \cite{everitt1989performance, zhao2005decentralized,maskery2009decentralized}. However, most existing work in this field concerns the design of Medium Access Control (MAC) protocols (a faster time scale than that of flow arrivals), and most often, channels may take two states only, busy or free. 



%In this framework, tenants must assign flows to channels or reject them outright, still avoiding conflicts. While this area is well-studied, a limitation of this framework is that channels typically take binary values (occupied or free) which is simpler what we're considering.






%{\bf Flow-level admission control.}
%The traditional framework for admission control in computer communication methods is dynamic channel assignment 

%The Best Arm dentification problem was introduced by \cite{audibert2010best} in the context of finding the single arm with greatest reward, and solved in the fixed confidence setting in terms of presenting an explicit problem dependent lower bound with a matching algorithm by \cite{garivier2016optimal}, using a theoretical framework developed in \cite{garivier2019explore}. Working in a fixed budget setting, \cite{locatelli2016} studied the problem of separating arms by whether their reward was greater or smaller than a threhold, while \cite{kaufmann2018sequential} studied the problem of identifying whether the smallest mean of a set of arms was smaller than a threshold. Further, \cite{garivier2018thresholding} studied the problem of finding the arm with reward closest to some given threshold, with or without assumptions of monotonicity on the arm rewards with respect to order. These problems carry great similarity to that of identifying admissible servers. Using game theoretic methods, \cite{degenne2019pure} ambitiously extended the general Best Arm Identification framework to the case with multiple correct answers, covering a vast array of problems. However, their lower bound is non-explicit, and their algorithm ``Sticky Track-and-Stop'' is often difficult to implement for non-gaussian arm reward distributions.

% {\bf DRL techniques}

%Machine learning has received considerable interest in the network control and management community \cite{du2020machine} \cite{boutaba2018comprehensive}. One field of particular interest, especially for 5G networks, is slice management \cite{ojijo2020survey} in terms of for example admission control and resource scaling. Below we review a number of recent works on slice admission control.

%A reinforcement-learning approach is studied to tackle the challenge of the admission control problem in multimedia networks in \cite{tong2000adaptive}. The challenge is to maximize network revenue  while simultaneously meeting quality of service constraints that forbid entry into certain states and use
%of certain actions. The admission control problem is modeled as a semi-Markov decision processes, and the reinforcement-learning approach is based on Q-learning. 


%In \cite{raza2019reinforcement} the authors propose a reinforcement-learning based approach for slice admission control with the objective of maximizing the profit of an infrastructure provider in presence of services with varying priorities and requirements (e.g. in terms of latency, capacity). The method learns how to maximize the revenue by admitting high revenue slice requests while minimizing the penalty by rejecting slices with a lower revenue expectation. A slice request is specified in terms of holding time, service priority, and number of resources required. The RL-agent is modeled as a stochastic policy network, based on a neural network.

%In \cite{sciancalepore2019rl} the authors propose a reinforcement learning-based slice broker with three main components; slice utilization forecasting, admission controller, and a slice scheduler. Of specific interest to this paper is the admission controller that receives a slice request defined by requirements in terms of resources, the expected lifetime, and the traffic class. The slice admission control is modelled as a multiple geometric knapsack problem with inputs on currently used resources and a forecast of upcoming utilization. The algorithm proposal is based on heuristics. 

%In \cite{bakri2021using} the authors develop and evaluate three reinforcement-learning approaches with the objective of balancing the network resource utilization and the network slice requirements in terms of quality of service for an infrastructure provider. The approaches builds upon Q-learning, deep Q-learning, and regret matching. \textcolor{red}{I cannot access the full paper and thus cannot determine if it is a model-free or model-based approach.}



%The work in \cite{millnert2018autosac} models the slice as a service chain of network functions that can scale based on momentary requirements. A fluid network queue model is used to approximate the service chain. The admission to the slice is considered per packet; admitted if the estimated queuing delay is lower than a threshold value determined by the service requirement policy.

%None of the above works consider the challenges addressed by this paper, namely the cost of sampling and transporting data from network elements to an admission-control agent. 



%{\bf Flow-level admission control.}


%{\bf Bandits.}

%{\bf DRL techniques}


==> Tech report version/Sections/3.Models.tex <==
\section{Models: Dynamics, Admission Control, and Measurement Costs}\label{sec:models}

This section presents our network model, and states our admission control problem. The network consists of $K$ slices of equal capacity.
%\footnote{The model and our results can be easily extended to account for heterogeneous slices.}. 
The network handles traffic {\it flows} or {\it services} generated by end users, and its resources are shared by many users. When a new flow is created, the slice tenant managing these users, or in other words the \emph{controller}, has no knowledge about the current traffic conditions on the various slices, but wishes to select a slice so that the performance guarantees of existing flows in the slice 
% Network operator or slice tenant? I think we're running into a fundamental issue here.
remains as high as possible. In this case, this translates to ensuring the loads of all slices remains below some \emph{threshold}. To determine which slice should handle the flow or whether the flow should be rejected, the controller has to measure the traffic intensity on slices. This measurement procedure induces a cost, such as power or bandwidth consumption, that the controller wishes to minimize. We describe this cost minimization problem in detail below, and an outline of the system is found in Figure \ref{fig:sliceadmissioncontrol}. In this figure, the slices are visualized as a chain of virtual network functions (VNFs) depicted as blue boxes, connected to radio over network links with a controller monitoring the network. The shaded areas correspond to the utilization level of the VNFs as consumed by a set of flows. In this case, the correct decision is for the controller to admit into Slice 1 as it is the only available slice.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.45\textwidth]{graphics/Network_slice_simple_model.png}
	\caption{Admission control in sliced networks.}
	\label{fig:sliceadmissioncontrol}
\end{figure}

\subsection{Packet-level dynamics and admission criteria}

Flows are assumed to generate packets according to a stationary process. When for a given slice, the set of accepted flows is fixed, we assume that the aggregate packet arrival process has statistics described, for simplicity, by a single parameter. Time is slotted, and this parameter is defined as the average number of packets arriving in one slot. In this paper, the processes might be Bernoulli (if the slot duration is very small), or Poisson (for the usual Poisson model at packet level in data networks), but extending the results to more sophisticated distributions is simple if so desired. 
%It will, however, be assumed that the process will belong to some exponential family. 
For slice $k\in [K]$, we denote by $\mu_k$ as the mean packet arrival rate per slot, fixed during a decision setting, and define $\boldsymbol{\mu}=(\mu_1,\ldots,\mu_K)$. $\mathbb{P}_{\boldsymbol{\mu}}$ (resp. $\mathbb{E}_{\boldsymbol{\mu}}$) denotes the probability distribution (resp. the expectation) of observations when the packet arrival rates are parametrized by $\boldsymbol{\mu}$. 

Assume that a user generates a new flow with known packet arrival rate $r$. Further assume that the current traffic in the network is described by $\boldsymbol{\mu}$. We consider scenarios where accepting the flow should be ideally decided based on $r$ and $\boldsymbol{\mu}$. This happens for example when we wish to guarantee that the average packet delay
%\footnote{We may wish to target some probabilistic guarantees for the delay, e.g., smaller than a maximum delay with some level of certainty. Considering such guarantees would lead to other kind of learning problems.}
of accepted flows remains smaller than a given threshold. For Poisson packet arrivals, the threshold $\gamma$ is obtained simply by plugging $r$, $\boldsymbol{\mu}$, the slice capacity, and packet size statistics in the M/G/1 Pollaczek--Khinchine formula. As a result, the flow should be ideally accepted in slice $k$ only if $\mu_k< \gamma$, in which case, we say that slice $k$ is {\it available}. The flow should be rejected if none of the slices is available. In this paper, when a new flow is created, $\boldsymbol{\mu}$ is unknown and has to be learnt. 

\subsection{Best slice identification problems}

The controller applies a joint measurement and decision strategy to decide whether a newly generated flow can be accepted and if so, on which slice. In each slot $t\ge 1$, we may measure for a selected slice, say $k$, the number of packets $X_k(t)$ handled by the slice in that slot.
%\footnote{A simple modification of the model can allow the user to probe several slices simultaneously.}. 
For example under the Poisson traffic assumption, the r.v. $X_k(t)$ are i.i.d. with Poisson distribution of unknown mean $\mu_k$. Now a joint measurement and decision strategy consists of three components:
\begin{itemize}
\item[(i)] {\it A sampling strategy.} It specifies, in each slot, the slice to measure. Measurements are taken once per slice and consider end-to-end load, rather than load in individual VNFs (as in Figure \ref{fig:sliceadmissioncontrol}). For $t\ge 1$, denote by $k_t$ and by $X_{k_t}(t)$ the slice probe in slot $t$ and the corresponding number of packets observed. Then $k_t$ depends on past observations, i.e., $k_t$ is ${\cal F}_{t-1}$-measurable where ${\cal F}_t$ is the $\sigma$-algebra generated by $(k_1,X_{k_1}(1),\ldots, k_t,X_{k_t}(t))$.
\item[(ii)] {\it A stopping rule.} It controls the end of the data acquisition phase and is defined as a stopping time $\tau$ with respect to the filtration $(\mathcal{F}_t)_{t\ge 1}$ such that $\mathbb{P}_{\boldsymbol{\mu}}(\tau < \infty) = 1$.
\item[(iii)] {\it A decision rule.} At the end of slot $\tau$, the algorithm returns a decision $\hat{k}(\tau)\in \{0,1,\ldots,K\}$, where $\hat{k}(\tau)=0$ means that the flow is rejected, and $\hat{k}(\tau)=k\ge 1$ is the selected available slice.  $\hat{k}(\tau)$ depends on all the observations made and is hence ${\cal F}_\tau$-measurable.
\end{itemize}

A correct decision is obtained when $\hat{k}(\tau)=0$ if there is no slice with load below the threshold, or when $\hat{k}(\tau)$ is an available slice. There may be multiple available slices, and we can further specify the admission criteria by refining the definition of a correct decision. It is not immediately obvious that any criterion is strictly better than one another, but we will consider algorithms pertaining to each of the following three criteria and compare them to one another. In all scenarios, we denote by ${\cal C}(\boldsymbol{\mu})\subset \{0,1,\ldots,K\}$ the set of correct answers given the server loads $\boldsymbol{\mu}$. We also define $\mu_\star = \min_k \mu_k$ as the smallest load between slices and $k_\star\in\arg\min_k\mu_k$ as the least loaded slice. Finally we let $k^\star \in \arg\max_{k:\mu_k< \gamma}\mu_k$ be the most loaded available slice, defined only when $\mu_\star<\gamma$.
\begin{enumerate}
	
	\item \setlength\parfillskip{0pt plus .75\textwidth}
	\setlength\emergencystretch{1pt} {\it Any available slice.} Under this criterion, we have ${\cal C}(\boldsymbol{\mu})=\{k: \mu_k< \gamma\}$ if $\mu_\star< \gamma$ and \linebreak ${\cal C}(\boldsymbol{\mu})=\{0\}$ otherwise.
\item {\it Packing slice.} Here, we wish to select the most loaded available slice, referred to as the {\it packing} slice. This choice allows us to get a minimum number of active slices, and in some scenarios where the service rates of incoming flows are heterogenous, to reduce the blocking rate. Under this criterion, ${\cal C}(\boldsymbol{\mu})=\{ k^\star \}$ if $\mu_\star< \gamma$ and ${\cal C}(\boldsymbol{\mu})=\{0\}$ otherwise and we denote $\mu^\star = \mu_{k^\star}$.
\item  {\it Least loaded slice.} Selecting the least loaded available slice is also a natural admission criterion, since it will tend to homogenize the loads of the slices, and hence ensure fairness (packet of the various flows experience similar delays) and low packet delay. Here, ${\cal C}(\boldsymbol{\mu})=\{k_\star\}$ if $\mu_\star< \gamma$ and ${\cal C}(\boldsymbol{\mu})=\{0\}$ otherwise. While superficially similar to the problem considered by \cite{garivier2018thresholding}, this criterion differs in the requirement that the slice be available which creates a discontinuity for loads near $\gamma$ and thereby disqualifies the methods considered in that~paper.
\end{enumerate}

Given one of the aforementioned admission criteria, we wish to design algorithms returning a correct answer with a fixed level of certainty. Note that since $\boldsymbol{\mu}$ is unknown and measurements are inherently noisy, it is impossible to surely get a correct answer. We fix $\delta>0$, and target $\delta$-PC ($\delta$-Probably Correct) algorithms, that is, algorithms which are guaranteed to return the correct answer with at least probability $1 - \delta$:

\begin{definition}[$\delta$-PC algorithms] A joint measurement and decision algorithm is $\delta$-PC if and only if for any $\boldsymbol{\mu}$, $\mathbb{P}_{\boldsymbol{\mu}}[\tau<\infty]=1$ and $\mathbb{P}_{\boldsymbol{\mu}}[\hat{k}(\tau)\notin {\cal C}(\boldsymbol{\mu})]\le \delta$.
\end{definition}

The objective is to devise a $\delta$-PC algorithm with minimal expected measurement cost or sample complexity $\mathbb{E}_{\boldsymbol{\mu}}[\tau]$ for the various envisioned admission criteria. 
  

\subsection{Induced flow-level dynamics}

While this paper mainly focuses on devising efficient measurement schemes, it is worth mentioning and studying the impact of the chosen admission criteria on the flow-level performance, i.e., on the flow blocking probabilities. To simplify the discussion below, we assume that the admission decisions are always correct, so that we can focus on the impact of the chosen admission criteria. The deviations caused by the fact that our algorithms may sometimes fail to output a correct decision are assessed numerically in section \ref{sec:num}.   

\smallskip
\noindent
{\it Homogenous flows.} When flows generate packets at the same rate, then all admission criteria lead to the same dynamics at flow-level (the process describing the number of ongoing flows) and hence the same blocking probability (given for example by one of Erlang formulas if flow arrivals are Poisson). In that case, it is best to choose the admission criteria with the minimum measurement cost.

\smallskip
\noindent
{\it Heterogenous flows.} When the flows have different rates, then the selected admission criterion impacts the flow-level dynamics and blocking probabilities. It has been shown that with heterogeneous flows, the steady-state distribution of the population of flows is sensitive to flow size distribution, arrival process and time scale \cite{bonald2003insensitive}, and we cannot analytically characterize the blocking rates. This difficulty arises essentially because with heterogenous flows, the network dynamics are not monotonic in any sense and not reversible \cite{kelly1979reversibility}. As a consequence, it is difficult to predict the behavior of any given admission controller.  We will investigate the trade-off achieved under different admission criteria between blocking probabilities and measurement costs only numerically (see Section \ref{sec:num}).
%, and we will therefore use admission criteria which either mimic popular admission controller or which suggest simple, measurement-cheap policies, and compare their blocking probabilities numerically in section \ref{sec:num}.



==> Tech report version/Sections/4.AnythingGoes.tex <==
\section{Identifying any Available Slice}\label{sec:anythinggoes}

With this first admission criterion, we wish to identify {\it any} available slice using a minimum number of measurements. This problem resembles the thresholding bandit problem \cite{locatelli2016}. In the latter, the decision maker needs to identify the set of {\it all} slices below the threshold, which is arguably easier since there is in this case a unique correct answer, see \cite{degenne2019pure} and \cite{garivier2021nonasymptotic} for a discussion. Our problem is also close to those addressed in  \cite{kaufmann2018sequential}, where the goal is to identify whether there exists a slice below the threshold (here, we wish to identify one such slice if any). 

%In the first approach, the agent is asked to first identify if any arm $k$ is available (has a load $\mu_k$ smaller than $\gamma$) and if so, to name \emph{one} available arm  without regard to order. Defining $k_\star$ to be the arm with lowest mean and $\mu_\star = \mu_{k_\star}$, on this problem, then, 
%%
%$$C(\mu) = \begin{cases}
%	\{k: \mu_k < \gamma\} & \text{if } \mu_\star < \gamma \\
%	\{Reject\} & \text{otherwise.}
%\end{cases} $$
% Maybe reference to SEQ lowest mean testing is unnecessary here? We are using Any Low Arm from Degenne et al anyway

%We define $d(\mu_1, \mu_2)$ to be the KL-divergence between two members of the same exponential family with means $\mu_1$ and $\mu_2$, respectively, and in particular $d_B(p, q)$ to be this KL-divergence when $p$ and $q$ are means of Bernoulli distributions. We define $k_\star$ to be the arm with lowest mean and $\mu_\star = \mu_{k_\star}$. Algorithms consist of a sampling rule $\{k_t(\mathcal{F}_{t-1})\}_{t=1}^\infty$ (where $\mathcal{F}_t$ is the filtration generated by events up to and including time $t$), a terminal decision rule $D$, and a stopping time $\tau_\delta$. We say that an algorithm is $\delta$-correct on $\mathcal{M}$ if, for all  $\nu \in \mathcal{M}$, a) the algorithm stops in finite time almost surely and b) outputs a correct answer to the question above with probability at least $1-\delta$

\subsection{Lower bound on the average measurement cost}

To identify a fundamental cost limit satisfied by any $\delta$-PC algorithm, one can leverage the classical change-of-measure arguments first introduced by \cite{lai1985} to derive regret lower bound in stochastic bandits, and then adapted in \cite{garivier2016optimal} to pure exploration problems in bandits. However, as recently discussed in \cite{degenne2019pure} and \cite{garivier2021nonasymptotic}, deriving sample complexity lower bounds is here complicated by the fact that there are multiple correct answers. 

We introduce the following notations. Let $\Lambda$ be the $(K-1)$-dimensional simplex $\Lambda=\{ w\in [0,1]^K: \sum_kw_k=1\}$. We denote by $d(\mu, \nu)$ the Kullback-Leibler divergence (KL-divergence) between two distributions parametrized by $\mu$ and $\nu$, respectively.  $d_B(\mu, \nu)$ denotes this KL-divergence in the case of Bernoulli distributions. In the sequel, to avoid pathological cases where one cannot identify an available slice even with an infinite number of measurements, we assume that $\mu_\star \neq \gamma$. The following result is a corollary of Theorem 1 in \cite{degenne2019pure} and provides a sample complexity lower bound for any of the three admission criteria. 

\begin{proposition} For any admission criteria, the sample complexity of any $\delta$-PC algorithm satisfies, for any $\mu$ such that $\mu_\star \neq \gamma$, $\mathbb{E}_\mu[\tau] \geq T(\mu)d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
		T(\mu)^{-1} =\max_{k \in {\cal C}(\mu)} \max_{{w} \in \Lambda} \inf_{\lambda: k \notin {\cal C}(\lambda)} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell}).
	\end{equation}
	\label{prop:GeneralLowerBound}
	\end{proposition}
	%

The above lower bound, defined by the {\it characteristic} time $T(\mu)$, is not explicit, and in general hard to compute. We may interpret this lower bound as follows. Let ${\cal  C}^\star(\mu)\subseteq {\cal C}(\mu)$ the set of maximizers over $k$ of $F(\mu,k)=\max_{{w} \in \Lambda} \inf_{\lambda: k \notin {\cal C}(\lambda)} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell})$. Slices in ${\cal  C}^\star(\mu)$ are the {\it easiest} correct answers to identify, and an optimal algorithm should sample as to output one of these slices. Identifying $k\in {\cal  C}^\star(\mu)$ is done with minimal sample complexity when the sampling rule realizes the allocation of slice draws defined by ${w}^\star(\mu, k) = \arg\max_{{w} \in \Lambda}F(\mu,w,k)$. The following proposition provides an explicit expression of the lower bound for the any-available-slice identification problem. 

\begin{proposition}
For the any-available-slice problem, we have, for any $k\in {\cal C}(\mu)$ and all $\ell\in [K]$,
\begin{equation}
w_\ell^\star(\mu, k) = \mathds{1}_{(k = 0)}\frac{d(\mu_\ell, \gamma)^{-1}}{\sum_{j=1}^{K}d(\mu_j, \gamma)^{-1}} + \mathds{1}_{(k=\ell)}.
	\label{eq:OptimalAnythingProportions}
	\end{equation}
%\begin{equation}
%w_k^\star(\mu, \ell) = \begin{cases}
%			\frac{(d(\mu_\ell, \gamma))^{-1}}{\sum_{j=1}^{K}(d(\mu_j, \gamma))^{-1}} & \text{if } k= 0 \ \ \text{(reject)},\\
%	\mathds{1}(\ell = k) & \text{otherwise.}
%\end{cases}
%	\label{eq:OptimalAnythingProportions}
%	\end{equation}
%	%
In particular, the sample complexity of any $\delta$-PC algorithm satisfies $\mathbb{E}_\mu[\tau] \geq T_1(\mu)d_B(\delta,1-\delta)$		
where
	%
	\begin{equation}
		T_1(\mu) = \begin{cases}
			d(\mu_\star, \gamma)^{-1} & \text{if } \mu_\star < \gamma, \\
			\sum_{j=1}^K d(\mu_j, \gamma)^{-1} & \text{otherwise.}
		\end{cases}
	\end{equation}
	\label{prop:AnythingLowerBound}
\end{proposition}

The proof of the above Proposition and those of the other results presented in this paper are postponed to the appendix. Note that in the any-available-slice problem, the easiest slices to identify are those with minimum load: 
\begin{equation}\label{eq:easy1}
{\cal C}^\star(\mu)=\left\{
\begin{array}{ll}
\{k: \mu_k=\mu_\star\} & \hbox{ if } \mu_\star<\gamma,\\
\{0\}& \hbox{ otherwise.}
\end{array}
\right.
\end{equation}
Further note that the optimal sampling rule suggested by the lower bound is {\it discountinuous}: if $\mu_\star < \gamma$,  it samples only slices with load $\mu_\star$, but if $\mu_\star > \gamma$ it samples all slices with different frequencies.

%\begin{proof}[Proof sketch] 
%	The proof logic closely follows that of \cite{kaufmann2018sequential}. If $\mu_\star > \gamma$, the agent needs to, individually, sample all arms and verify that their mean is greater than $\gamma$. If, on the other hand, $\mu_\star < \gamma$, it suffices to verify that any particular arm has mean smaller than $\gamma$. The most efficient way, for an oracle, to accomplish this is to sample only $k_\star$. With these facts in mind, the proposition follows from the fundamental lemma in \cite{garivier2019explore}. The full proof can be found in Appendix \ref{appx:LowerBoundProofs}.
%\end{proof}






\subsection{Track-and-Stop algorithm}
%% TODO: Decide whether to keep Multiple correct answers framework, and if so, describe it, or to rewrite with different framework.

Next, we describe the Track-and-Stop (\textsc{TaS}) algorithm, a generic algorithm that will be instantiated for the three identification problem, and establish its asymptotic optimality (when $\delta$ approaches 0) for the any-available-slice problem.

\medskip
\noindent
{\it Sampling rule.} The sample complexity lower bound and its interpretation provide the design principle of the sampling rule. In this paper, we follow the Track-and-Stop framework developed in \cite{garivier2016optimal} for best arm identification problem in bandits. In this framework, extended to our problem, the $t$-th measured slice is chosen as follows. $\mu$ is estimated by its sample mean $\hat{\mu}(t-1)$ from the $(t-1)$-th first measurements. $\hat{\mu}(t-1)$ then replaces $\mu$ in $w^\star({\mu},k)$ and ${\cal C}^\star(\mu)$, i.e., these are approximated by $\hat{w}^\star(t,k):=w^\star(\hat{\mu}(t-1),k)$ and $\hat{\cal C}(t):={\cal C}^\star(\hat{\mu}(t))$, respectively. Finally, we select a target slice\footnote{The subscript 'E' stands for 'Easiest'.} $k_E(t)$ from $\hat{\cal C}^\star(t)$, and sample the slice $k_t$ to measure using the proportions $\hat{w}^\star(t,k_E(t))$. The way $k_E(t)$ is selected from $\hat{\cal C}^\star(t)$ matters in general, and here, we always select the slice with minimal index. The algorithm described above works as long as we can make sure that $\hat{\mu}(t)$ converges to $\mu$ a.s.. To this aim, the sampling rule includes a {\it forced exploration} phase: after $t$ measurements, slices that have not been measured more than $\sqrt{t}$ times are measured. If the algorithm is not in a forced exploration phase, it tracks the allocation $\hat{w}^\star(t,k_E(t))$, i.e., it measures the slice $k_t\in \arg\max_k t\hat{w}^\star_k(t,k_E(t))-N_k(t-1)$, where $N_k(t-1)$ is the number of times $k$ has been measured so far. Finally note that the sampling rule depends on the functions $\mu\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$. For the any-available-slice problem, these are given by (\ref{eq:OptimalAnythingProportions}) and (\ref{eq:easy1}), respectively.

\medskip
\noindent
{\it Stopping rule.} The stopping rule we use is classical and relies on a similar stopping criterion as in all previously devised pure exploration algorithms. Specifically, it is based on the Generalized Likelihood Ratio (GLR) statistics $Z_{k,k'}(t)$ evaluating the probabilities that given the observations, the targeted correct answer is $k=k_E(t)$ or $k'$, see details in \cite{garivier2016optimal} and \cite{degenne2019pure}. We stop when these GLR are large enough. The resulting statistical test can summarized by comparing $\inf_{\lambda: \hat{k}(t) \notin \mathcal{C}(\lambda)} \sum_{k=1}^K N_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$ to an exploration threshold $f_\delta(t)$ appropriately chosen.  

\medskip
\noindent
{\it Decision rule.} When the algorithm stops measuring after $\tau$ measurements, it returns the slice $k_E(\tau)$. The pseudo-code of the algorithm is presented in Algorithm \ref{alg:TaS}. There, $N(t)$ denotes the vector counting the number of times each slice has been measured up to time $t$ (such that $\sum_{k=1}^K N_{k}(t) = t$). 

%To utilize the lower bounds in practice, we will employ versions of ``Track-and-Stop'' with D-tracking \cite{garivier2016optimal}, so named for the use of a \emph{tracking} sample rule. Let $\hat{\mu}(t)$ be the sample mean of each arm at time $t$ and let $N(t)$ be the vector counting the number of times each arm has been pulled up to time $t$ (such that $\sum_{k=1}^K N_{k}(t) = t$). We will assume that we have access to an oracle $\hat{w}^\star(\mu)$ which for any answer $\ell \in \mathcal{C}(\hat{\mu}(t))$ and any given time $t$ can calculate the optimal proportions as $\hat{w}(t) = \hat{w}^\star(\hat{\mu}(t), \ell)$. Such an oracle will generally employ lower bound results such as that in \ref{prop:AnythingLowerBound}. Further, we denote by $\hat{k}(t)$ the algorithm's output at time $t$, which will be generated by a \emph{best arm rule} $\hat{k}^\star(\mu)$. Let $f_\delta(t)$ be a stopping function. We describe the algorithm as presented by \cite{degenne2019pure} in Algorithm \ref{alg:TaS}.

\begin{algorithm}[t]
	\caption{Track-and-Stop (\textsc{TaS})}
	\label{alg:TaS}
	\begin{algorithmic}

		% I don't like the notation for the empirical best arm rule... Is there anything better?		
		%\Require Best arm rule $\hat{k}^\star: \mathcal{M} \to [K]$
		%\Require Oracle weight function $\hat{w}^\star:\mathcal{M} \times [K] \to \Lambda$
		%Oracle functions $w^\star(\mu,k)$ and ${\cal C}^\star(\mu)$
		\State {\bf Input:} Oracle functions $(\mu,k)\mapsto w^\star(\mu,k)$ and $\mu\mapsto {\cal C}^\star(\mu)$
		\State {\bf Initialization:} $\hat{\mu}(0) = 0$, $N(0) = 0$
		\For{$t=1,...$}
		\State ${k}_E(t)\leftarrow  \min {\cal C}^\star(\hat{\mu}(t-1))$
		\State $Q(t)\leftarrow \inf_{\lambda: {k}_E(t) \notin \mathcal{C}(\lambda)} \sum_{k=1}^K N_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$
		\If{$Q(t) > f_\delta(t)$}
		\State Stop and return ${k}_E(t)$
		\EndIf
		\State $\hat{w}(t)\leftarrow  {w}^\star(\hat{\mu}(t-1), {k}_E(t))$
		\If{$\exists k: N_{k}(t-1) < \sqrt{t}$}
		\State $k_t \leftarrow \arg\min_k N_{k}(t-1)$
		\Else
		\State $k_t \leftarrow \arg \max_k t \hat{w}_{k}(t) - N_{k}(t-1)$
		\EndIf
		\State Measure slice $k_t$ and observe $X_{k_t}(t)$
		\State  $N(t) \leftarrow N(t-1) + {\bf e}_{k_t}$
		\State $\hat{\mu}(t)\leftarrow \hat{\mu}(t-1) + \frac{1}{N_{k_t}(t)}(X_{k_t}(t) - \hat{\mu}_{k_t}(t-1)) {\bf e}_{k_t}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

%The idea behind Algorithm \ref{alg:TaS} is to \emph{track} the empirical weights $\hat{w}(t)$ and sample as if they were the true oracle weights, stopping when the probability of making an error is sufficiently small. It is applicable on many problems in its current form, but needs explicit methods to calculate $\hat{k}^\star$ and $\hat{w}^\star$ before implementation.
%For the problem of identifying any available slice, we select $\hat{k}^\star(\mu) = k_\star \mathds{1}_{(\mu_\star < \gamma)} $. Further, for the weight function $\hat{w}^\star$ we use $w^\star$ as defined in equation \eqref{eq:OptimalAnythingProportions}. 

\medskip
The following theorem, proved leveraging results from \cite{degenne2019pure}, establishes the asymptotic (as $\delta$ goes to 0) optimality of \textsc{TaS} for the any-available-slice problem, up to a factor 2. 

\begin{theorem}
Let \textsc{TaS} be instantiated for the any-available-slice problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalAnythingProportions}) and (\ref{eq:easy1}), respectively. Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k_\star$ is unique,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\mathbb{E}_\mu[\tau]}{d_B(\delta,1-\delta)} \leq 2T_1(\mu).
	\end{equation}
	\label{the:AlgResults}
\end{theorem}

We conclude this section by remarking that for $\mu$ such that $k_\star$ is not unique, we would need to add a component to the algorithm to avoid the oscillation of $k_E(t)$ between these slices with minimal load. This is done in \cite{degenne2019pure} by introducing a {\it sticky} component to the algorithm. We could follow this idea, but for simplicity and clarity of the paper, prefer to restrict our attention to the cases where $k_\star$ is unique. 



%This is a direct consequence of Theorem 11 in \cite{degenne2019pure} since the \emph{Any available slice} problem is equivalent to the \emph{Any Low Arm} problem in the framework of that paper. Notably, since we by previous measurement cost bounds showed that
%%
%$$\liminf_{\delta \to 0} \frac{\E{\tau_\delta}}{\log(1/\delta)} \geq T_1(\mu)$$
%%
%for any $\delta$-correct algorithm, this implies that \textsc{TaS} is asymptotically optimal. This does not translate to optimality in moderate confidence regions, but it does give some confidence in this choice of algorithm when the confidence level is high.




==> Tech report version/Sections/5.Packing.tex <==
\section{Identifying the Packing Slice}\label{sec:packing}

For the second admission criterion, the objective is to identify $k^\star$, the packing slice (if it exists). Recall that if $\mu_\star<\gamma$, $k^\star=\arg\max_{k:\mu_k< \gamma} \mu_k$. For simplicity, we will restrict our attention to slice loads $\mu$ such that the packing slice is unique when it exists. The identification problem slightly resembles the dose ranging problem addressed for Gaussian arms in \cite{garivier2018thresholding}, but there, the objective is to find the arm with the reward the closest to a given threshold -- not necessarily below, as in our case.   



%In the second approach, the agent is asked to identify the (assumed to be unique) \emph{packing} arm $k^\star$ with the greatest mean $\mu^\star < \gamma$, so that for all arms $k\neq k^\star$, either $\mu_k < \mu^\star$ or $\mu_k > \gamma$. This is useful for admission control since it allows us to ``pack'' services into slices, potentially leaving room for future demanding services.

\subsection{Lower bound on the average measurement cost}

As for the any-available-slice problem, we can derive lower bounds on the average measurement cost satisfied by any $\delta$-PC algorithm. To state these bounds, we distinguish two cases: (i) when $\mu_\star<\mu^\star<\gamma$ (which means that there exists a packing slice and that it is different from the slice with minimum load); and (ii) when either $\mu_\star > \gamma$ (the correct answer is 0) or $\mu_\star=\mu^\star<\gamma$ (there is a unique available slice). 

For the first case only, we introduce the following notations. For any $\mu, \nu$, $\alpha\in [0,1]$, let $I_\alpha(\mu, \nu) = \alpha d(\mu, \alpha \mu + (1-\alpha)\nu) + (1-\alpha) d(\nu, \alpha \mu + (1-\alpha)\nu)$ be a weighted symmetrization of the KL divergence with weight $\alpha$. Define the information function of slice $k$ in relation to slice $k^\star$ as $g_k(x) = (1+x)I_{\frac{1}{1+x}}(\mu^\star, \mu_k)$. Further, let $x_k^\star(y) = g_k^{-1}(y)$, and $x_{k^\star}^\star(y)=1$ for all $y$ by convention. Let $\mu_k'(y) = \frac{\mu^\star + \mu_a x_k^\star(y)}{1 + x_k^\star(y)}$, and finally define the function $F_P$ by
\begin{equation}
		F_P(y)= \sum_{k:\mu_k< \mu^\star} \frac{d(\mu^\star, \mu_k'(y))}{d(\mu_k, \mu_k'(y))}.
	\end{equation} 
The next proposition provides an explicit expression of the sample complexity lower bound for the problem of identifying the packing slice. Its proof starts from the results of Proposition \ref{prop:GeneralLowerBound}, and can be found in appendix. 

\begin{proposition}
Consider a $\delta$-PC algorithm with sample complexity $\tau$.\\
(i) Assume that $\mu$ satisfies $\mu_\star < \mu^\star < \gamma$. Let $z^\star = \min(d(\mu^\star, \gamma), y^\star)$ where $y^\star$ is the unique solution to the equation $F_P(y) = 1$ ($y^\star$ and $z^\star$ are well defined). Then, $\E[\mu]{\tau} \geq T_2(\mu)d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
		T_2(\mu) = \sum_{k: \mu_k > \mu^\star} d(\mu_k, \gamma)^{-1} +
		\frac{1}{z^\star}\sum_{k:\mu_k<\gamma} x_k^\star(z^\star).
	\end{equation}
	%
	Furthermore, we have, for any $k \in [K]$,
	%
	\begin{equation}
		w_k^\star(\mu, k^\star) =\frac{1}{T_2(\mu)} \left( \frac{x_k^\star(z^\star)\mathds{1}_{(\mu_k < \gamma)}}{z^\star} + \frac{\mathds{1}_{(\mu_k > \gamma)}}{d(\mu_k, \gamma)} \right).
		% \begin{cases}
		%	\frac{x_a(z^\star)}{z^\star T_2(\mu)}	&	\text{if } \mu_k < \mu^\star \\
		%	\frac{1}{z^\star T_2(\mu)} 			&	\text{if } k = k^\star \\
		%	\frac{1}{d(\mu_k, \gamma)T_2(\mu)}	&	\text{otherwise.}
		%\end{cases}
		\label{eq:OptimalPackingProportions}
	\end{equation}
	%
(ii) Assume that $\mu$ satisfies $\mu_\star > \gamma$ or $\mu_\star = \mu^\star < \gamma$. Then, $\E[\mu]{\tau} \geq T_2(\mu)d_B(\delta,1-\delta)$ where
	%
	\begin{equation}
		T_2(\mu) = \sum_{k=1}^K d(\mu_k, \gamma)^{-1}.
	\end{equation}
	%
	Furthermore, we have, for any $k \in [K]$ and any $\ell \in \mathcal{C}(\mu)$ (so $\ell = 0$ if $\mu_\star > \gamma$ and $\ell = k^\star$ if $\mu_\star = \mu^\star$), 	%
	\begin{equation}
		w_k^\star(\mu, \ell) =\frac{d(\mu_k,\gamma)^{-1}}{T_2(\mu)}.
		% \begin{cases}
		%	\frac{x_a(z^\star)}{z^\star T_2(\mu)}	&	\text{if } \mu_k < \mu^\star \\
		%	\frac{1}{z^\star T_2(\mu)} 			&	\text{if } k = k^\star \\
		%	\frac{1}{d(\mu_k, \gamma)T_2(\mu)}	&	\text{otherwise.}
		%\end{cases}
		\label{eq:OptimalPackingProportionsDegenCase}
	\end{equation}
\label{prop:PackingLowerBound}
\end{proposition}


%\begin{proof}[Proof sketch]
%	The full proof can be found in Appendix \ref{appx:LowerBoundProofs}. In general, there are three ways to create an alternate problem $\lambda$ where $k^\star$ is no longer optimal
%	
%	\begin{enumerate}
%		\item For some arm $k$ with $\mu_k > \gamma$, modify this arm such that $\lambda_k < \gamma$.
%		\item For some arm $k$ with $\mu_k < \mu^\star$, modify this arm and $k^\star$ such that $\lambda_k > \lambda_{k^\star}$. 
%		\item Modify $k^\star$ such that $\lambda_{k^\star} > \gamma$.
%	\end{enumerate}
%	
%	First, we note that arms such that $\mu_k > \gamma$ are only treated in condition 1. Further, there is no need to compare them to $k^\star$ directly, since any perturbation that makes $\lambda_k < \gamma$ suffices to confuse the agent. Thus, the agent needs to verify that all these arms are greater than $\gamma$, which from the thresholding means problem we know requires to pull arm $k$ at least $d_B(\delta,1-\delta)/d(\mu_k,\gamma)$ times. This leads to the first summand in $T_2$, and we will not need to consider these arms any more. 
%	
%	Similarly, the third condition tells us that arm $k^\star$ must be pulled at least $d_B(\delta,1-\delta)/d(\mu^\star,\gamma)$ times. The second condition adds a wrinkle to this, however. The second condition can be seen as solving a best arm identification problem for all arms $k$ with $\mu_k < \gamma$. From \cite{garivier2016optimal}, we know that this implies that for all arms, they need to be pulled $n_k$ times and further, for symmetry reasons, the quantity $g_k(n_k/n_{k^\star})$ is identical for all arms $k \neq k^\star$. Furthermore, we also know that, in the unconstrained case, this quantity is identical to $y^\star$ as given in the proposition. It can be shown that if $y^\star \leq d(\mu^\star,\gamma)$, the arm $k^\star$ will be sufficiently pulled by a best arm identification algorithm and so, we have the second case in the second term of $T_2$. However, if this is not the case we still find that the quantities $g_k(n_k/n_{k^\star})$ are equal but that they are also equal to $d(\mu^\star, \gamma)$. This leads to the first case.
%	
%	
%\end{proof}

Remember that we made the assumption that $k^\star$ is unique when it exists. When this is not the case, the lower bound of Proposition \ref{prop:PackingLowerBound} would suggest an infinite sample complexity. We can circumvent this difficulty by accepting \emph{overlapping hypotheses} \cite{garivier2021nonasymptotic}, i.e., we can require the algorithm to output a slice $k$ with mean $\mu^\star - \varepsilon \leq \mu_k \leq \mu^\star$ with probability $1 - \delta$ for some tolerance threshold $\varepsilon > 0$. For clarity of the exposition, we omit the rather lengthy theoretical analysis required to bound the sample complexity of such algorithms.


\subsection{Track-and-Stop algorithm}
Under the assumption of a unique packing arm $k^\star$, we can use \textsc{TaS} (Algorithm \ref{alg:TaS}) to solve the packing-slice identification problem. To this aim, we instantiate the algorithm using: 
\begin{equation}\label{eq:css}
{\cal C}^\star(\mu) = \left\{
\begin{array}{ll}
\{ k^\star\} &\hbox{ if }\mu_\star<\gamma,\\
\{0\}&\hbox{ otherwise,}
\end{array}
\right.
\end{equation}
 and the weight function $w^\star$ defined in  (\ref{eq:OptimalPackingProportions}) and (\ref{eq:OptimalPackingProportionsDegenCase}) depending on the case.

\begin{theorem}
Let \textsc{TaS} be instantiated for the packing-slice identification problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalPackingProportions}),  (\ref{eq:OptimalPackingProportionsDegenCase}) and (\ref{eq:css}). Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k^\star$ is unique when it exists,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\E[\mu]{\tau}}{d_B(\delta,1-\delta)} \leq 2T_2(\mu).
	\end{equation}
	\label{the:PackingAlg}
\end{theorem}


==> Tech report version/Sections/6.MinimumLoad.tex <==
\section{Identifying the Least Loaded Available Slice}\label{sec:minimumload}

For the last admission criterion, we wish to identify the least loaded slice $k_\star$ provided it is below the threshold $\gamma$. This criterion is sometimes preferable to ensure that the load is evenly distributed between slices. The corresponding identification problem is related to the classical Best Arm Identification problem \cite{garivier2016optimal} with the important difference that here if the load of $k_\star$ is above the threshold $\gamma$, the correct decision is to reject the flow. We assume again to simplify the presentation that $k_\star$ is unique.

\subsection{Lower bound on the average measurement cost}

To state the lower bound, we distinguish two cases: (i) when $\mu_\star<\gamma$ (the correct answer is $k_\star$); (ii) when $\mu_\star>\gamma$ (the correct answer is $0$). For the first case only, we will use the following notation. Define $h_k(x):=(1+x)I_{\frac{1}{1+x}}(\mu_\star, \mu_k)$, $x_{\star, k}(y) := h_k^{-1}(y)$ (with, again, $x_{\star, k_\star}(y)= 1$ for all $y$) and $\mu_k''(y) := \frac{\mu_\star + \mu_k x_{\star, k}(y)}{1 + x_{\star, k}(y)}$  and finally $F_{ML}$ is the function
%
\begin{equation}
	F_{ML}(y)= \sum_{k:\mu_k> \mu_\star} \frac{d(\mu_\star, \mu_k''(y))}{d(\mu_k, \mu_k''(y))}.
\end{equation}  
$F_{ML}$ is defined whenever there exist at least two arms (in any other case, the problem is trivial) and is monotonic.

\begin{proposition}		
Consider a $\delta$-PC algorithm with sample complexity $\tau$.\\
(i) Assume that $\mu$ satisfies $\mu_\star < \gamma$. Let $z_\star = \min(d(\mu_\star, \gamma), y_\star)$ where $y_\star$ is the unique solution to the equation $F_{ML}(y) = 1$ ($y_\star$ and $z_\star$ are well defined). Then we have $\E[\mu]{\tau} \geq T_3(\mu)d_B(\delta,1-\delta)$ where 
	\begin{equation}
		T_3(\mu) = \frac{1}{z_\star} \sum_{k = 1}^K x_{\star, k}(z_\star).
	\end{equation}
	%
	Furthermore, we have, for all $k \in [K]$,
	%
	\begin{equation}
		w_k^\star(\mu ,k_\star) = \frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}.
		%\begin{cases}
		%	\frac{1}{z_\star T_3(\mu)} &	\text{if } k=k_\star \\
		%	\frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}		& \text{otherwise.}
		%\end{cases}
	\label{eq:OptimalMinimumProportions}
	\end{equation}
(ii) Assume that $\mu$ satisfies $\mu_\star > \gamma$. Then, we have $\E[\mu]{\tau} \geq T_3(\mu)d_B(\delta,1-\delta)$ where 
	\begin{equation}
		T_3(\mu) = \sum_{k = 1}^K d(\mu_k, \gamma)^{-1}.
	\end{equation}
	%
	Furthermore,  we have, for all $k \in [K]$,	%
	\begin{equation}
		w_k^\star(\mu,0) = \frac{d(\mu_k, \gamma)^{-1}}{T_3(\mu)}. 
		%\begin{cases}
		%	\frac{1}{z_\star T_3(\mu)} &	\text{if } k=k_\star \\
		%	\frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}		& \text{otherwise.}
		%\end{cases}
		\label{eq:OptimalMinimumProportionsDegenCase}
	\end{equation}
	\label{prop:MinimumLowerBound}
\end{proposition}

%\begin{proof}[Proof sketch]
%	The set of confusing problems $\neg k_\star$ can be written as the union of $\Lambda_2 = \{\lambda \in \mathcal{M}: \exists a \neq _\star: \lambda_a < \lambda_{k_\star} \}$ and $\Lambda_3 = \{\lambda \in \mathcal{M}: \lambda_{k_\star} > \gamma \}$. The rest of the analysis is completely analogous to the one concerning $\Lambda_2$ and $\Lambda_3$ in the proof of Proposition \ref{prop:PackingLowerBound} (see Appendix \ref{appx:LowerBoundProofs}).
%\end{proof}

The expressions of the sample complexity lower bounds in the packing-slice and least-slice identification problems enjoy a similar form. However, they are quantitatively often very different. Indeed, $\mu^\star$ is often much closer to $\gamma$ than $\mu_\star$, and as a result, $d(\mu^\star, \gamma) \ll d(\mu_\star, \gamma)$ and identifying the packing-slice requires much more measurements. 

\subsection{Track-and-Stop algorithm}

Under the assumption of a unique least loaded slice $k_\star$, we can use \textsc{TaS} (Algorithm \ref{alg:TaS}) to solve the least-loaded-slice identification problem. To this aim, we instantiate the algorithm using: 
\begin{equation}\label{eq:css2}
{\cal C}^\star(\mu) = \left\{
\begin{array}{ll}
\{ k_\star\} &\hbox{ if }\mu_\star<\gamma,\\
\{0\}&\hbox{ otherwise,}
\end{array}
\right.
\end{equation}
 and the weight function $w^\star$ defined in  (\ref{eq:OptimalMinimumProportions}) and (\ref{eq:OptimalMinimumProportionsDegenCase}) depending on the case.

\begin{theorem}
Let \textsc{TaS} be instantiated for the least-loaded-slice identification problem with input functions $(\mu,k)\mapsto w^\star({\mu},k)$ and $\mu\mapsto{\cal C}^\star(\mu)$ given by (\ref{eq:OptimalMinimumProportions}),  (\ref{eq:OptimalMinimumProportionsDegenCase}) and (\ref{eq:css2}). Select an exploration rate equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies: for any $\mu$ such that $k_\star$ is unique,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\E[\mu]{\tau}}{d_B(\delta,1-\delta)} \leq 2T_3(\mu).
	\end{equation}
	\label{the:MinimumAlg}
\end{theorem}



==> Tech report version/Sections/7.NumericalExperiments.tex <==
\section{Simulations}\label{sec:num}

We have run simulations to illustrate the performance of our joint measurement and decision strategies under the various admission criteria. To do so, we fixed the system load and invested the measurement costs of our algorithm using the different admission criteria. Then, we investigated to what extent the constraints are violated and compared the sampling efficiency with a naive sampling algorithm. Finally, we studied the dynamical behavior of the system given that different admission criteria gives rise to different admission control behavior.

\subsection{Packet level dynamics and local optimality}
We studied a system with $K=8$ slices of equal slice resources. The flows we are interested in are services in the range of Conversational Voice, Conversational Video and Live Gaming. Conversational Voice has a packet frequency of about $50$ packets/s \cite{cisco2016voip}. Conversational video sends a bitrate of about 1500 kbps \cite{ibm20xxbitrate} and has a packet size of about 1500 bytes \cite{sengupta2017movidiff} which translates to a packet frequency of about 125 packets per second. Finally, Live Gaming has a typical packet interarrival time of $40$ ms which translates to $25$ packets/s \cite{che2012packet}. In this first case of study, we therefore assumed that each slice could hold 24 flows,
that each UE sent, on average, $50$ packets per second and that in each measurement we measured the number of packets sent during a slot of length $20$ ms \footnote{$20$ ms is chosen arbitrarily to have each UE send about $1$ packet per slot, but we can see similar results with other slot lengths.}. Thus, the admission threshold $\gamma$ was fixed equal to $\gamma = 24 \times 50 \times 0.02=24$ packets/slot, corresponding to a bit rate of 14 Mbps.

The traffic intensity $\mu$ on each slice was generated randomly from a truncated uniform multinomial distribution according to the following parameters:

\begin{enumerate}
	\item The total load is fixed according to the scenarios
	\begin{itemize}
		\item \emph{Low load} with an average of $17$ packets/slot/slice,
		\item \emph{Medium load} with an average of $23$ packets/slot/slice and
		\item \emph{High load} with an average of $30$ packets/slot/slice.
	\end{itemize}  
	\item The probability of any unit load being assigned to a slice is uniform over slices.
	%\item If the packing slice or least loaded available slice is not unique, the load is reinstantiated until both are unique. This was to avoid unnecessarily high variance in sampling complexity, but did introduce a small bias.
\end{enumerate}

\begin{table*}[t]
	\centering
	\begin{tabular}{r|ccc|ccc|ccc}
		& \multicolumn{3}{c|}{{\bf Any-available-slice}}  & \multicolumn{3}{c|}{{\bf Packing-slice}} & \multicolumn{3}{c}{{\bf Least-loaded-slice}} \\
		Scenario 
		&
		\textsc{TaS} & Uniform & Lower bound & \textsc{TaS} & Uniform & Lower bound & \textsc{TaS} & Uniform & Lower bound \\
		\hline
		Low load	 & 12.2 & 27.7 & 0.843 & 808 & 2800 & 245 & 390 & 1020 & 139 \\
		Medium load & 28.4 & 105 & 2.88  & 1790 & 5480 & 571 & 565 & 1350 & 180\\
		High load & 571 & 3522 & 92.6 & 897 & 3640 & 261 & 897 & 2310 & 290\\
		
	\end{tabular}
	\caption{Measurement costs in slots (averaged over 100 runs -- confidence intervals are not shown due to space constraints but are typically small, with radius of the order of $5\%$ of mean).}
	\label{tab:PacketResults}
\end{table*}

Note that since the intensity is generated by a multinomial distribution, it only takes integer values. In the first and second scenarios, an available slice is always available by the pigeon hole principle, and so, we expected a greater discrepancy between the different admission criteria in measurement cost. In the third scenario, an available slice is not always available and so we expected the difference to be smaller.
We implemented \textsc{TaS} in Python 3.7 under the three admission criteria, and compared their performance to that of a naive algorithm using the same stopping and decision rules but with a sampling rule picking slices in a round-robin manner. This benchmark is useful as it allows us to see the impact of only our intelligent sampling rule, removing the impact of confidence levels and other performance guarantees. The level of confidence for the stopping rule was fixed to $\delta = 0.01$. Each algorithm was tested on 100 independent runs, and in each run the traffic intensity $\boldsymbol{\mu}$ was regenerated. The results are shown in Table \ref{tab:PacketResults}, including the averaged lower bounds from Section \ref{sec:AbbrTheory} for comparison.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{graphics/confidence_ratio.eps}
	\caption{The measurement costs as a function of the confidence parameter $\delta$. The red lines depict the measurement cost and lower bound while the blue line represents the ratio between the two.}
	\label{fig:confidence_ratio}
\end{figure}


Observe that the problems with different admission criteria have different difficulties. As expected, the any-available-slice criterion leads to a much lower measurement cost, except for the high load scenario where there is often no or a single available slice. In all scenarios, \textsc{TaS} significantly outperforms a naive algorithm using uniform sampling: the improvements in the measurement cost are by a factor $2$ to $8$ on all problems. \textsc{TaS} measurement costs are not so close to the lower bound, an effect we attribute to the moderate confidence level \linebreak of $\delta = 0.01$. To verify this, we evaluated the measurement cost, as compared to the lower bound, for a variety of values of $\delta$ in the range $[10^{-7}, 10^{-2}]$ with the packing-slice criterion and high load. These costs and lower bounds, along with the ratio between the two are shown in Figure \ref{fig:confidence_ratio}. We see that the measurement cost increases sub-linearly with $\log(1/\delta)$ and that it converges to approximately $1.8$ when $\delta \to 0$, which is consistent with Theorem \ref{the:AlgResults}.
%It might seem surprising to get a lower bound of 0.84 in the low load scenario for the any-available-slice criterion, but remember that a single measurement yields a Poisson r.v. with mean often as low as $8$ or $10$ as compared to the threshold of $24$ and hence already brings a lot of information.





\subsection{Measurement costs and blocking rates averaged over flow dynamics}
Next, we account for our simulations on flow-level dynamics. Flows were generated according to a Poisson process of intensity $\bar{\lambda}$ (flows per time unit). When a flow arrives, its packet arrival rate $r$ was chosen uniformly at random in $\{1, ..., 10\}$ per slot. We used $K=3$ slices, each of capacity 15.5 packets per slot. A flow of rate $r$ can be accepted on a slice $k$ only if $\mu_k < \gamma = 15.5 -r$ (the admission threshold depends on the rate $r$). Flow durations were exponentially distributed with mean of 1 time unit. Note that the time unit is assumed to be much larger than the duration of a slot, so that the population of flows can be assumed to be fixed over a slot when measurements were conducted. Overall, the {\it load} of the system used was $\rho = {\bar{\lambda}\bar{r}\over 15.5 K}$ where $\bar{r}=5.5$ is the average flow rate. For \textsc{TaS}, the confidence level $\delta$ was set to $0.01$. We examined all admission criteria: any-available-slice, packing-slice and least-loaded-slice. For the measurement cost, we include the lower bounds $T_i(\mu)$  from Section \ref{sec:AbbrTheory}, averaged over the flow states $\mu$ seen by the controller across the experiment.  The results can be found in Figure \ref{fig:AlgorithmComparison}.

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{graphics/uniform_distribution_blocking_3_slices.eps}
		\caption{Overall blocking probability}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{graphics/uniform_distribution_elephant_3_slices.eps}
		\caption{Blocking probability of high-rate flows}
	\end{subfigure}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=\textwidth]{graphics/uniform_distribution_measure_3_slices_w_expected.eps}
		\caption{Number of measurements}
	\end{subfigure}
	\caption{Flow-level performance under the various admission criteria and \textsc{TaS}. (a) Blocking probability averaged over all flows vs. load; (b) Blocking probability of flows with the highest rate (10) vs. load; (c) Measurement cost vs. load (solid lines report the performance of \textsc{TaS}, and dashed lines our averaged lower bounds).}
\label{fig:AlgorithmComparison}
\end{figure*}

Figure \ref{fig:AlgorithmComparison} highlights the trade-off between blocking probabilities and measurement costs. The any-available-slice criterion offers the lowest measurement cost but this comes at the expense of a higher blocking probability. The overall blocking probability is 2 to 5 times greater under the any-available-slice criterion than under the packing-slice criterion. The latter offers the lowest blocking rates but has a high measurement cost -- almost 10 times greater compared to the any-available-slice criterion. It seems that the least-loaded-slice criterion yields the best trade-off between blocking rates and measurement costs.

Another important result, not presented in these figures, is that during our experiments, there was no occasion during which the system was overloaded. This suggests that \textsc{TaS} is more conservative compared to what the targeted confidence level $\delta = 0.01$ imposes.



==> Tech report version/Sections/8.Conclusions.tex <==
\section{Conclusions}\label{sec:conclusion}

In this paper, we investigated the problem of admission control in network slicing where before admitting or rejecting a flow, the slice utilization of several slices needs to be measured. Inspired by Best Arm Identification methods, we designed a framework to allow for robust admission control with confidence guarantees. We applied this framework to devise optimal joint measurement and admission schemes realizing three different admission criteria. We verified, using simulations, the optimality of our algorithms as compared to the lower bounds and showed their advantage over naive measurement methods. In this paper, we assumed that the unknown parameters, driving the admission decisions and implicitly learnt by our algorithms, just dictate the loads of the slices. In practice, in real sliced networks, there might be other types of uncertainty (e.g. unknown flow rate or unknown slice capacity), and we plan to extend our methods and results to deal with these additional uncertainties.


%
% 
%For future work, we aim to expand our methods to real sliced networks as well as expand the framework to allow information to be carried over between decisions.




%We showed how three admission criteria can be adapted in this framework, showed fundamental measurement cost bounds for these algorithms and adapted algorithms to meet these bounds while maintaining confidence guarantees, analytically proving our results. We verified in experiments that these guarantees are met and showed both the advantage of our methods over naive measurement methods as well as how they interacted with flow level dynamics to create a trade-off between blocking probability, fairness and measurement cost. For future work, we aim to expand our methods to real sliced networks as well as expand the framework to allow information to be carried over between decisions.

==> Tech report version/Sections/A.LowerBoundProof.tex <==
\section{Lower bound proofs}\label{appx:LowerBoundProofs}

\subsection{Proof of Propositions \ref{prop:RejectLowerBound} and \ref{prop:AnythingLowerBound}}
Recall that $\Lambda$ is the simplex of dimension $(K - 1)$. For any correct answer $\ell \in \mathcal{C}(\boldsymbol{\mu})$, denote by $\text{Alt}(\ell) := \{ \boldsymbol{\lambda}: \ell \notin \mathcal{C}(\boldsymbol{\lambda}) \}$, and denote by $D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) := \sum_{k=1}^Kw_kd(\mu_k,\lambda_k)$.
By Theorem 1 in \cite{degenne2019pure}, any $\delta$-PC algorithm must fulfill $\E[\boldsymbol{\mu}]{\tau} \geq T(\boldsymbol{\mu})d_B(\delta, 1 - \delta)$ where
%
$$
T(\boldsymbol{\mu})^{-1} = \max_{{w} \in \Lambda} \max_{\ell \in \mathcal{C}(\boldsymbol{\mu})}\inf_{\boldsymbol{\lambda}: \ell \in Alt(\boldsymbol{\lambda})} \sum_{k=1}^K w_k d(\mu_k, \lambda_k).
$$
 We therefore wish to solve the max-min problem
%
$$
\boldsymbol{w}^\star(\boldsymbol{\mu}) \in \arg\max_{\boldsymbol{w} \in \Lambda} \max_{\ell \in \mathcal{C}(\boldsymbol{\mu})} \inf_{\boldsymbol{\lambda} \in \text{Alt}(\ell)} D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}).
$$
%
%We will use the framework of ``Pure exploration with multiple correct answers'' \cite{degenne2019pure}. In Theorem 1 of this paper, it  is stated that our Proposition is true iff $T_1(\boldsymbol{\mu}) = D(\boldsymbol{\mu})^{-1}$ with $D(\boldsymbol{\mu}) = \max_{i \in i^\star(\boldsymbol{\mu})} \max_{{\bf w} \in \Delta_K} \inf_{\lambda \in \neg i} \sum_{k=1}^K w_k d(\mu_k, \lambda_k)$. Here $i^\star$ is the set of correct answers, which in our case is all arms $a$ with mean $\mu_a < \gamma$ if such an arm exists, and rejection otherwise. Further $\Delta_K$ is the simplex of dimension $K$ and $\neg i$ is the set of all bandit problems on which arm $i$ is not optimal.

We begin with the case $\mu_\star > \gamma$. Then $\mathcal{C}(\boldsymbol{\mu}) = \{0\}$ by definition of our admission criteria. We have that $\text{Alt}(0) = \{\boldsymbol{\lambda}:\exists k \in [K]: \lambda_k < \gamma\}$, and from this set, we can restrict ourselves to studying only $\boldsymbol{\lambda}^{(k)}$ such that $\lambda_{m}^{(k)}(\nu) = \nu \mathds{1}_{(m=k)} + \mu_m\mathds{1}_{(m \neq k)}$ with $\nu < \gamma$ (only a single arm $k$ is changed compared to $\boldsymbol{\mu}$). Indeed, for any instance $\boldsymbol{\lambda} \in \text{Alt}(\boldsymbol{\mu})$ and any weights $\boldsymbol{w} \in \Lambda$, there exists $k$ and $\nu$ such that $D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) \geq D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}^{(k)}(\nu))$. 
 %Then $i^\star$ has only the unique element of rejecting the incoming service. Further, $\neg i$ contains all problems $\lambda$ where $\exists a: \mu_a' < \gamma$. We can restrict ourselves to studying only problems $\lambda ^{(a)}$ where a single arm $a$ is changed such that $\lambda_b^{(a)} = \mu_b\ \forall b \neq a$ and $\lambda_{(a)} = \gamma$, as any other problem $\lambda in \neg i$ will have a greater value of
%\begin{equation}
%	D({\bf w}, \mu, \lambda) :=\sum_{k=1}^K w_k d(\mu_k, \lambda_k)
%\end{equation}
It follows that for any $\boldsymbol{w} \in \Lambda$,  $\inf_{\boldsymbol{\lambda} \in \text{Alt}(\ell)}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) = \min_{k\in[K]} D(\boldsymbol{w},\boldsymbol{\mu},\boldsymbol{\lambda}^{(k)}(\gamma)) = \min_{k\in[K]}w_kd(\mu_k, \gamma)$. We note then that for maximizing $\boldsymbol{w}=\boldsymbol{w}^\star(\boldsymbol{\mu})$, it must be true that $D(\boldsymbol{w}^\star(\boldsymbol{\mu}),\boldsymbol{\mu},\boldsymbol{\lambda}^{(k)}(\gamma)) =D(\boldsymbol{w}^\star(\boldsymbol{\mu}),\boldsymbol{\mu},\boldsymbol{\lambda}^{(m)}(\gamma))\ \forall k \in [K],m \in [K]$. Adding the condition $\sum_{k=1}^Kw_k = 1$, this yields a linear equation system which is easily solved with
%
\begin{equation}
	w^\star_k(\boldsymbol{\mu}, 0) = \frac{d(\mu_k, \gamma)^{-1}}{\sum_{j=1}^K d(\mu_j, \gamma)^{-1}}
\end{equation}
%
and therefore, by the above lower bound, $T_0(\boldsymbol{\mu}) = \sum_{k=1}^K d(\mu_k, \gamma)^{-1}$, which concludes this case. However, this case also extends easily to the Packing-slice and Least-Loaded-slice problem, since it is simple to show that the set of confusing problems $\text{Alt}(0)$ remains the same for these.

Next, we study the any-available-slice case with $\mu_\star < \gamma$. Take any arm $\ell \in \mathcal{C}(\boldsymbol{\mu})$,  with $\mu_\ell < \gamma$. For this case, $\text{Alt}(\ell)$ are all problems $\boldsymbol{\lambda}$ such that $\lambda_\ell > \gamma$. Similarly as before, it is easy to see that $ \inf_{\boldsymbol{\lambda} \in \text{Alt}(\ell)} D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) =D({\bf w}, \boldsymbol{\mu}, \boldsymbol{\lambda}^{(\ell)}(\gamma)) = w_\ell d(\mu_\ell,\gamma)$. Furthermore, this expression is maximized under $\boldsymbol{w} \in \Lambda$ and $\ell \in \mathcal{C}(\boldsymbol{\mu})$ by $\boldsymbol{w}^\star(\boldsymbol{\mu})$ with $w^\star_k(\boldsymbol{\mu}) = \mathds{1} (k = \ell)\ \forall k \in [K]$ and $\ell = k_\star(\boldsymbol{\mu})$. Therefore, we see that Proposition \ref{prop:AnythingLowerBound} holds with $T_1(\boldsymbol{\mu}) = d(\mu_\star, \gamma)^{-1}$ as above. This concludes this case and the proof.

\subsection{Proof of Proposition \ref{prop:PackingLowerBound}}
		We will assume that $\mu_\star <\mu^\star < \gamma$ (for the case $\mu_\star = \mu^\star < \gamma$, refer to the proof of Propositions \ref{prop:RejectLowerBound} and \ref{prop:AnythingLowerBound}). In this case, $\mathcal{C}(\boldsymbol{\mu}) = \{k^\star(\boldsymbol{\mu})\}$, with $k^\star(\boldsymbol{\mu})$ unique by hypothesis. We notice that $\text{Alt}(k^\star(\boldsymbol{\mu}))$ can be written as the union of three sets, $\text{Alt}(k^\star(\boldsymbol{\mu})) \subseteq A_1 \cup A_2 \cup A_3$ where
	
	
	\begin{enumerate}
		\item $A_1 := \{\boldsymbol{\lambda}: \exists k: \mu_k > \gamma,\ \lambda_k < \gamma\}$,
		\item $A_2 := \{\boldsymbol{\lambda}: \exists k: \mu_k < \mu^\star, \lambda_{k^\star(\boldsymbol{\mu})} < \lambda_k < \gamma \}$,
		\item $A_3 := \{\boldsymbol{\lambda}: \lambda_{k^\star(\boldsymbol{\mu})} > \gamma \}$.
	\end{enumerate}
Hence,	%
	$$
	\inf_{\boldsymbol{\lambda} \in \text{Alt}(k^\star(\boldsymbol{\mu}))}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) = \inf_{\boldsymbol{\lambda} \in A_1 \cup A_2 \cup A_3}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}).
	$$
	%
	We will first find the value of $\inf_{\boldsymbol{\lambda} \in A_i}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda})$ for $i \in \{1,2,3\}$. This value is
	
	\begin{enumerate}
		\item for $A_1$, $\min_{k: \mu_k > \gamma} w_k d(\mu_k, \gamma)$,
		\item for $A_2$, $\min_{k: \mu_k < \mu^\star}: w_{k^\star(\boldsymbol{\mu})}I_{w_{k^\star(\boldsymbol{\mu})}/(w_k + w_{k^\star(\boldsymbol{\mu})})}(\mu^\star, \mu_k)$, % TODO: Define I or rewrite this
		\item  and for $A_3$, $w_{k^\star(\boldsymbol{\mu})}d(\mu^\star, \gamma)$.
	\end{enumerate}
	
	Let $D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))$ be the minimum of these three expressions. Since the sets of modified arms are non-overlapping between $A_1$ and $A_2 \cup A_3$, we see that for each arm $k$ with $\mu_k > \gamma$ the expression $w_kd(\mu_k, \gamma)$ must be equal and identical to $D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))$ for any maximizing $\boldsymbol{w}$, and thereby, for these arms $w^\star_k(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu})) = D^\star(\boldsymbol{w}^\star(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu})), \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))d(\mu_a, \gamma)^{-1}$.
	
	 For $A_2$, the best proportions $w^\star_k$ are known from Best Arm Identification problems \cite{garivier2016optimal} and can be found as $w^\star_k = \frac{x_{k,k^\star(\boldsymbol{\mu})}(y^\star) D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))}{y^\star}$ for all $k$ with $\mu_k < \gamma$, where $x_{k,k^\star(\boldsymbol{\mu})}(y)$ and $y^\star$ are defined in the proposition.
	
	Now, if $y^\star \leq d(\mu^\star, \gamma)$ then $\frac{D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu}))) d(\mu^\star, \gamma)}{y^\star} \geq D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))$ and so these proportions maximize the expression $\min_{\boldsymbol{\lambda} \in A_2  \cup A_3} D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda})$. 
	
	If instead $y^\star > d(\mu^\star, \gamma)$, by convexity of $D^\star(\cdot, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))$, we see that $w_{k^\star(\boldsymbol{\mu})}=\frac{D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))}{d(\mu_1, \gamma)}$ is maximizing and so, since the expression $I_{w_{k^\star(\boldsymbol{\mu})}/(w_a + w_{k^\star(\boldsymbol{\mu})})}(\mu^\star, \mu_a)$ must be identical to $\frac{D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))}{w_{k^\star(\boldsymbol{\mu})}}$ for all arms $k$ with $\mu_k < \gamma$, we obtain $w^\star_k = \frac{D^\star(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))}{d(\mu_1, \gamma) x_{k,k^\star(\boldsymbol{\mu})}(d(\mu^\star, \gamma))}{d(\mu^\star, \gamma)}$.
	In summary, recalling that $z^\star = \min(d(\mu^\star, \gamma), y^\star)$, we find that $w^\star_k(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu})) = \frac{D^\star(\boldsymbol{w}^\star(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu})), \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu}))) x_{k,k^\star(\boldsymbol{\mu})}(z^\star)}{z^\star}\ \forall k:\ \mu_k < \gamma$.
	
	Finally, we make use of the fact that $\sum_{k} w_ak= 1$, and find that 
	%
	\begin{align*}
		D^\star(\boldsymbol{w}^\star&(\boldsymbol{\mu}), \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu}))) =\\
		&= \left(\sum_{k: \mu_k > \gamma}d(\mu_k, \gamma)^{-1} + \frac{1}{z^\star} \sum_{k:\mu_k< \gamma} x_{k,k^\star(\boldsymbol{\mu})}(z^\star) \right)^{-1}.
	\end{align*}
	%
	But since these proportions $\boldsymbol{w}^\star(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu}))$ are maximizing, we obtain by Theorem 1 in \cite{degenne2019pure} that any $\delta$-PC algorithm must be sampled in expectation at least $T_2(\boldsymbol{\mu})d_B(\delta,1-\delta)$ times, with $T_2(\boldsymbol{\mu}) = D^\star(\boldsymbol{w}^\star(\boldsymbol{\mu}, k^\star(\boldsymbol{\mu})), \boldsymbol{\mu}, \text{Alt}(k^\star(\boldsymbol{\mu})))^{-1} = \sum_{k: \mu_k > \gamma } d(\mu_k, \gamma)^{-1} + \frac{1}{z^\star}  \sum_{k:\mu_k< \gamma} x_{k,k^star}(z^\star)$. This concludes the proof.
	
\subsection{Proof of Proposition \ref{prop:MinimumLowerBound}}
We recall that $\mathcal{C}(\boldsymbol{\mu}) = \{k_\star(\boldsymbol{\mu})\}$ with $k_\star(\boldsymbol{\mu})$ unique by hypothesis. As in the proof of Proposition \ref{prop:PackingLowerBound}, we note that $\text{Alt}(k_\star(\boldsymbol{\mu})) \subseteq A_2 \cup A_3$ with $A_2 = \{\boldsymbol{\lambda}: \exists k: \lambda_k < \lambda_{k_\star(\boldsymbol{\mu})}\}$ and $A_3 = \{\boldsymbol{\lambda}: \lambda_{k_\star(\boldsymbol{\mu})} > \gamma\}$, and furthermore
%
$$
\inf_{\boldsymbol{\lambda} \in \text{Alt}(k^\star(\boldsymbol{\mu}))}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) = \inf_{\boldsymbol{\lambda} \in  A_2 \cup A_3}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}).
$$
%
Next, like before we find that $\inf_{\boldsymbol{\lambda} \in A_2}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) = \min_{k: \mu_k>\mu_\star}w_{k_\star(\boldsymbol{\mu})} I_{w_{k_\star(\boldsymbol{\mu})}/(w_k + w_{k_\star(\boldsymbol{\mu})})}(\mu_\star, \mu_k)$ and\\ $\inf_{\boldsymbol{\lambda} \in A_3}D(\boldsymbol{w}, \boldsymbol{\mu}, \boldsymbol{\lambda}) = w_{k_\star(\boldsymbol{\mu})} d(\mu_\star, \gamma)^{-1}$.

As in the proof of Proposition \ref{prop:PackingLowerBound}, if $y_\star \leq d(\mu_\star, \gamma)$, then the optimal proportions are those of a Best Arm Identification problem and $\boldsymbol{w}^\star_k(\boldsymbol{\mu}, k_\star(\boldsymbol{\mu})) = \frac{x_{k,k_\star(\boldsymbol{\mu})}(y_\star)}{y_\star T_3(\boldsymbol{\mu})}$ with $T_3(\boldsymbol{\mu}) := \frac{1}{y_\star}\sum_{k=1}^K x_{k,k_\star(\boldsymbol{\mu})}(y_\star)$ for all $k$ with $y_\star$ and $x_{k,k_\star(\boldsymbol{\mu})}$ defined as in Section \ref{sec:AbbrTheory}.

Otherwise, by convexity of $D(\cdot, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu}))))$ and by $w_{k_\star(\boldsymbol{\mu})}d(\mu_\star, \gamma) = D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu})))$, we find that $w^\star_{k_\star(\boldsymbol{\mu})}(\boldsymbol{\mu}) = d(\mu_\star, \gamma)^{-1} D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu})))$. Since then $d(\mu_\star, \gamma)^{-1} D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu})))g(w_k/w_{k_\star(\boldsymbol{\mu})}) = D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu})))$ it follows that $w^\star_k(\boldsymbol{\mu}) = w^\star_{k^\star(\boldsymbol{\mu})}(\boldsymbol{\mu})x_{\star,k}(d(\mu_\star, \gamma))$ for all $k$. Utilizing $\sum_{k=1}^Kw_k = 1$ and defining in this case $T_3(\boldsymbol{\mu}) :=D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(k_\star(\boldsymbol{\mu})))^{-1}= \sum_{k=1}^K d(\mu_\star, \gamma)^{-1}x_{\star,k}(d(\mu_\star, \gamma))$, Equation \eqref{eq:OptimalMinimumProportions} follows. The remainder of Proposition \ref{prop:MinimumLowerBound} follows from Theorem 1 in \cite{degenne2019pure}.
	
	
	

==> Tech report version/Sections/AbbreviatedTheory.tex <==
\section{Best arm identification in admission control}\label{sec:AbbrTheory}

To devise $\delta$-PC algorithms with minimal measurement cost for each admission criterion, we first derive lower bounds on this cost. For a given criterion, we show that the lower bound is the value of an optimization problem, whose solution specifies the optimal measurement process (it characterizes the numbers of times an algorithm with minimal cost should measure each slice before stopping). We then develop algorithms whose sampling and stopping rules perform this optimal measurement process.  


%As is common in Best arm identification, our strategy will be to show lower bounds for sample complexity for all three criteria followed by an algorithm which we show match this lower bound.

\subsection{Lower bounds}

\noindent
{\bf Notations.} To state the lower bounds, we introduce the following notations. Let $\Lambda$ be the $(K-1)$-dimensional simplex $\Lambda=\{ \boldsymbol{w}\in [0,1]^K: \sum_kw_k=1\}$. We denote by $d(a,b)$ the Kullback-Leibler divergence (KL-divergence) between two distributions of the same one-parameter exponential family, parameterized by means $a$ and $b$, respectively. $d_B(a,b)$ denotes this KL-divergence in the case of Bernoulli distributions. In the sequel, to avoid pathological cases where one cannot identify an available slice even with an infinite number of measurements, we assume that $\mu_\star \neq \gamma$. Furthermore, we introduce the information deviation function as $g_{j,k}(x) = d(\mu_k, (\mu_k+x\mu_j)/(1+x)) + x d(\mu_j,  (\mu_k+x\mu_j)/(1+x))$ and its inverse $x_{j,k}(y) = g_{j,k}^{-1}(y)$. 
% TODO: Clarify this sentence
%The information deviation function $g_{j,k}$ describes the information distance between two unknown slices when the ratio of sampling is $x$, found by examining the worst case, and the inverse function $x_{j,k}$ represents the ratio a candidate arm $j$ is sampled compared to a target arm $k$ when the information deviation is exactly $y$. 
We use this to introduce the equilibrium function for a set of candidate arms $\mathcal{S}$ and a target arm $k$
$$F_k(y;\mathcal{S}) = \sum_{j \in \mathcal{S}}\frac{d(\mu_k, (\mu_k + x_{j,k}(y)\mu_j)/(1+x_{j,k}(y)))}{d(\mu_j, (\mu_k + x_{j,k}(y)\mu_j)/(1+x_{j,k}(y)))}.$$
%
\begin{comment}
	The following result is a corollary of Theorem 1 in \cite{degenne2019pure} and provides a sample complexity lower bound for any of the three admission criteria. 
	
	\begin{proposition} 
	For any admission criteria, the sample complexity of any $\delta$-PC algorithm satisfies, for any $\mu$ such that $\mu_\star \neq \gamma$, $\mathbb{E}_\mu[\tau] \geq T(\mu)d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
	T(\mu)^{-1} =\max_{k \in {\cal C}(\mu)} \max_{{w} \in \Lambda} \inf_{\boldsymbol{\mu}: k \notin {\cal C}(\lambda)} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell}).
	\end{equation}
	\label{prop:GeneralLowerBound}
	\end{proposition}
	%
The above lower bound, defined by the {\it characteristic} time $T(\mu)$, is not explicit, and in general hard to compute. We may interpret this lower bound as follows. 
\end{comment}
Let ${\cal  C}^\star(\boldsymbol{\mu})\subseteq {\cal C}(\boldsymbol{\mu})$ be the set of maximizers over $k$ of $\max_{\boldsymbol{w} \in \Lambda} \inf_{\boldsymbol{\lambda}: k \notin {\cal C}(\boldsymbol{\lambda})} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell})$. Following the interpretation in \cite{degenne2019pure}, slices in ${\cal  C}^\star(\boldsymbol{\mu})$ are the {\it easiest} correct answers to identify, and an optimal algorithm should output one of these slices. 

\noindent
{\bf Lower bounds and the optimal measurement process.} Following the approach developed in \cite{garivier2016optimal}, we identify the cost lower bounds, as well as the corresponding optimal fractions of time each slice should be measured. These fractions, denoted by $\boldsymbol{w}^\star\in \Lambda$, depend on whether there is an available slice and on the admission criterion.  The following propositions are established in Appendix \ref{appx:LowerBoundProofs}.   
%, and identifying $k\in {\cal  C}^\star(\boldsymbol{\mu})$ is done with minimal sample complexity when the sampling rule realizes these optimal proportions defined by $\mathbf{w}^\star(\boldsymbol{\mu}) = \arg\max_{\mathbf{w} \in \Lambda}\max_{k \in {\cal C}(\boldsymbol{\mu})}\inf_{\boldsymbol{\lambda}: k \notin {\cal C}(\boldsymbol{\lambda})} \sum_{\ell=1}^K w_\ell d(\mu_{\ell},\lambda_{\ell})$. The following propositions provide an explicit expression of the lower bound for our three admission criteria. 

\begin{proposition} {\bf [No available slice]}
For all three criteria, if $\mathcal{C}(\boldsymbol{\mu})= \{0\}$ (there is no available slice), then any $\delta$-PC algorithm fulfills $\E[\boldsymbol{\mu}]{\tau} \geq T_0(\boldsymbol{\mu})d_B(\delta,1-\delta)$ where
	%
	$$
	T_0(\boldsymbol{\mu}) = \sum_{k = 1}^K d(\mu_k, \gamma)^{-1}.
	$$
	The optimal measurement process is given by, for all $k$, 
	%\begin{equation*}
		$w^\star_k(\boldsymbol{\mu}) = \frac{d(\mu_k, \gamma)^{-1}}{T_0(\boldsymbol{\mu})}$.
	%\end{equation*}
	\label{prop:RejectLowerBound}
\end{proposition}

\begin{proposition} {\bf [Any-available-slice]} For the any-available-slice problem with $\mathcal{C}(\boldsymbol{\mu}) \neq \{0\}$, any $\delta$-PC algorithm fulfills $\E[\boldsymbol{\mu}]{\tau} \geq T_1(\boldsymbol{\mu})d_B(\delta,1-\delta)$
	with
	%
	$
	T_1(\boldsymbol{\mu}) = d(\mu_\star,\gamma)^{-1}.
	$\\
	%
	The optimal measurement process is given by, for all $k$,
	%\begin{equation}
		$w_k^\star(\boldsymbol{\mu}) = \mathds{1}_{(k = k^\star)}$.
		%\label{eq:OptimalAnythingProportions}
	%\end{equation}
	\label{prop:AnythingLowerBound}
\end{proposition}

\begin{proposition} {\bf [Packing-slice]} For the packing-slice problem with $\mathcal{C}(\boldsymbol{\mu}) \neq \{0\}$, define $\mathcal{S}_{P} = \{j: \mu_j < \mu^\star\}$ and $z^\star = \min(d(\mu^\star, \gamma), y^\star)$ where $y^\star$ is the unique solution to the equation $F_{k^\star}(y;\mathcal{S}_{P}) = 1$ ($y^\star$ and $z^\star$ are well defined). Any $\delta$-PC algorithm fulfills $\E[\boldsymbol{\mu}]{\tau} \geq T_2(\boldsymbol{\mu})d_B(\delta,1-\delta)$ where 
	%
	\begin{equation}
		T_2(\boldsymbol{\mu}) = \sum_{k: \mu_k > \mu^\star} d(\mu_k, \gamma)^{-1} +
		\frac{1}{z^\star}\sum_{k:\mu_k<\gamma} x_{k,k^\star}(z^\star).
	\end{equation}
	%
	The optimal measurement process is given by, for all $k$,
	%
	\begin{equation}
		w_k^\star(\boldsymbol{\mu}) =\frac{1}{T_2(\boldsymbol{\mu})} \left( \frac{x_{k,k^\star}(z^\star)\mathds{1}_{(\mu_k < \gamma)}}{z^\star} + \frac{\mathds{1}_{(\mu_k > \gamma)}}{d(\mu_k, \gamma)} \right).
		% \begin{cases}
			%	\frac{x_a(z^\star)}{z^\star T_2(\mu)}	&	\text{if } \mu_k < \mu^\star \\
			%	\frac{1}{z^\star T_2(\mu)} 			&	\text{if } k = k^\star \\
			%	\frac{1}{d(\mu_k, \gamma)T_2(\mu)}	&	\text{otherwise.}
			%\end{cases}
		\label{eq:OptimalPackingProportions}
	\end{equation}
	%

	\label{prop:PackingLowerBound}
\end{proposition}

\begin{proposition} {\bf [Least-loaded-slice]} For the least-loaded-slice problem with $\mathcal{C}(\boldsymbol{\mu}) \neq \{0\}$, define $\mathcal{S}_{LL} = \{j: \mu_j > \mu_\star\}$ and $z_\star = \min(d(\mu_\star, \gamma), y_\star)$ where $y_\star$ is the unique solution to the equation $F_{k_\star}(y; \mathcal{S}_{LL}) = 1$ ($y_\star$ and $z_\star$ are well defined). Any $\delta$-PC algorithm fulfills $\E[\boldsymbol{\mu}]{\tau} \geq T_3(\boldsymbol{\mu})d_B(\delta,1-\delta)$ where 
	\begin{equation}
		T_3(\boldsymbol{\mu}) = \frac{1}{z_\star} \sum_{k = 1}^K x_{k, k_\star}(z_\star).
	\end{equation}
	%
	The optimal measurement process is given by, for all $k$,
	%
	\begin{equation}
		w_k^\star(\boldsymbol{\mu}) = \frac{x_{k,k_\star}(z_\star)}{z_\star T_3(\boldsymbol{\mu})}.
		%\begin{cases}
			%	\frac{1}{z_\star T_3(\mu)} &	\text{if } k=k_\star \\
			%	\frac{x_{\star, k}(z_\star)}{z_\star T_3(\mu)}		& \text{otherwise.}
			%\end{cases}
		\label{eq:OptimalMinimumProportions}
	\end{equation}

	\label{prop:MinimumLowerBound}
\end{proposition}



\subsection{Track-and-Stop algorithm}
%% TODO: Decide whether to keep Multiple correct answers framework, and if so, describe it, or to rewrite with different framework.

Next, we describe the Track-and-Stop (\textsc{TaS}) algorithm, a generic algorithm that will be instantiated for the three admission criteria, and establish its asymptotic optimality (when $\delta$ approaches 0).

\medskip
\noindent
{\it Sampling rule.} The measurement cost lower bounds and the corresponding optimal measurement process provide the design principle of the sampling rule. We follow the Track-and-Stop framework developed in \cite{garivier2016optimal}: the sampling rule is designed so as to track the optimal fractions $\boldsymbol{w}^\star(\boldsymbol{\mu})$ of time each slice should be measured. Here $\boldsymbol{\mu}$ is unknown, and hence, for the $t$-th measurement, we track $\hat{\boldsymbol{w}}^\star(t):=\boldsymbol{w}^\star(\hat{\boldsymbol{\mu}}(t-1))$ instead, where $\hat{\boldsymbol{\mu}}(t-1)$ are the estimated slice loads from the $(t-1)$-th first measurements. The algorithm will work as long as we can make sure that $\hat{\boldsymbol{\mu}}(t)$ converges to $\boldsymbol{\mu}$ almost surely. To this aim, the sampling rule includes a {\it forced exploration} phase: after $t$ measurements, slices that have not been measured more than $\sqrt{t}$ times are measured. 
If the algorithm is not in a forced exploration phase, it tracks the allocation $\hat{\boldsymbol{w}}^\star(t)$, i.e., it measures the slice $k_t\in \arg\max_k t\hat{w}^\star_k(t)-n_k(t-1)$, where $n_k(t-1)$ is the number of times $k$ has been measured so far. Finally note that the sampling rule depends on the functions $\boldsymbol{\mu}\mapsto \boldsymbol{w}^\star({\boldsymbol{\mu}})$ specified by Propositions \ref{prop:RejectLowerBound} - \ref{prop:MinimumLowerBound} for the various admission criteria.


% ${\cal C}^\star(\boldsymbol{\mu})$, i.e., these are approximated by $\hat{\mathbf{w}}^\star(t):=\mathbf{w}^\star(\hat{\boldsymbol{\mu}}(t-1))$ and $\hat{\cal C}(t):={\cal C}^\star(\hat{\boldsymbol{\mu}}(t))$, respectively. Finally, we select a target slice\footnote{The subscript 'E' stands for 'Easiest'.} $k_E(t)$ from $\hat{\cal C}^\star(t)$, and sample the slice $k_t$ to measure using the proportions $\hat{\mathbf{w}}^\star(t)$. The way $k_E(t)$ is selected from $\hat{\cal C}^\star(t)$ matters in general, and here, we always select the slice with minimal index. 



% For the any-available-slice problem, these are given by (\ref{eq:OptimalAnythingProportions}) and (\ref{eq:easy1}), respectively.

\medskip
\noindent
{\it Stopping rule.} The stopping rule we use relies on a similar stopping criterion as in all previously devised pure exploration algorithms. Specifically, it is based on the Generalized Likelihood Ratio (GLR) statistics $Z_{k,k'}(t)$ evaluating the probabilities that given the observations, the targeted correct answer is $k=k_E(t)$ or $k'$, see details in \cite{garivier2016optimal} and \cite{degenne2019pure}. We stop when these GLR are large enough. The resulting statistical test can summarized by comparing $Q(t):=\inf_{\boldsymbol{\lambda}: \hat{k}(t) \notin \mathcal{C}(\boldsymbol{\lambda})} \sum_{k=1}^K n_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$ to an exploration threshold $f_\delta(t)$ appropriately chosen.  

\medskip
\noindent
{\it Decision rule.} When the algorithm stops measuring after $\tau$ measurements, it returns the slice $k_E(\tau)$. The pseudo-code of the algorithm is presented in Algorithm \ref{alg:TaS}. There, $\mathbf{n}(t)$ denotes the vector counting the number of times each slice has been measured up to time $t$ (such that $\sum_{k=1}^K n_{k}(t) = t$). 


\begin{algorithm}[t]
	\caption{Track-and-Stop (\textsc{TaS})}
	\label{alg:TaS}
	\begin{algorithmic}
		
		% I don't like the notation for the empirical best arm rule... Is there anything better?		
		%\Require Best arm rule $\hat{k}^\star: \mathcal{M} \to [K]$
		%\Require Oracle weight function $\hat{w}^\star:\mathcal{M} \times [K] \to \Lambda$
		%Oracle functions $w^\star(\mu,k)$ and ${\cal C}^\star(\mu)$
		\State {\bf Input:} Oracle functions $\boldsymbol{\mu}\mapsto \mathbf{w}^\star(\boldsymbol{\mu})$ and $\boldsymbol{\mu}\mapsto {\cal C}^\star(\boldsymbol{\mu})$
		\State {\bf Initialization:} $\hat{\boldsymbol{\mu}}(0) = 0$, $\mathbf{n}(0) = 0$
		\For{$t=1,...$}
		\State ${k}_E(t)\leftarrow  \min {\cal C}^\star(\hat{\boldsymbol{\mu}}(t-1))$
		\State $Q(t)\leftarrow \inf_{\boldsymbol{\lambda}: {k}_E(t) \notin \mathcal{C}(\boldsymbol{\lambda})} \sum_{k=1}^K n_{k}(t-1) d(\hat{\mu}_{k}(t-1), \lambda_k)$
		\If{$Q(t) > f_\delta(t)$}
		\State Stop and return ${k}_E(t)$
		\EndIf
		\State $\hat{\mathbf{w}}(t)\leftarrow  \mathbf{w}^\star(\hat{\boldsymbol{\mu}}(t-1))$
		\If{$\exists k: n_{k}(t-1) < \sqrt{t}$}
		\State $k_t \leftarrow \arg\min_k n_{k}(t-1)$
		\Else
		\State $k_t \leftarrow \arg \max_k t \hat{w}_{k}(t) - n_{k}(t-1)$
		\EndIf
		\State Measure slice $k_t$ and observe $X_{k_t}(t)$
		\State  $\mathbf{n}(t) \leftarrow \mathbf{n}(t-1) + {\bf e}_{k_t}$
		\State $\hat{\boldsymbol{\mu}}(t)\leftarrow \hat{\boldsymbol{\mu}}(t-1) + \frac{1}{n_{k_t}(t)}(X_{k_t}(t) - \hat{\mu}_{k_t}(t-1)) {\bf e}_{k_t}$
		\EndFor
	\end{algorithmic}
\end{algorithm}

%The idea behind Algorithm \ref{alg:TaS} is to \emph{track} the empirical weights $\hat{w}(t)$ and sample as if they were the true oracle weights, stopping when the probability of making an error is sufficiently small. It is applicable on many problems in its current form, but needs explicit methods to calculate $\hat{k}^\star$ and $\hat{w}^\star$ before implementation.
%For the problem of identifying any available slice, we select $\hat{k}^\star(\mu) = k_\star \mathds{1}_{(\mu_\star < \gamma)} $. Further, for the weight function $\hat{w}^\star$ we use $w^\star$ as defined in equation \eqref{eq:OptimalAnythingProportions}. 

\medskip
The following theorem, proved leveraging results from \cite{degenne2019pure} in Appendix \ref{appx:UpperBoundProofs}, establishes the asymptotic (as $\delta$ goes to 0) optimality of \textsc{TaS} for the any-available-slice problem, up to a factor 2. 

\begin{theorem}
	Let \textsc{TaS} be instantiated for any of our admission criteria with input functions $\boldsymbol{\mu}\mapsto \mathbf{w}^\star({\boldsymbol{\mu}})$  given by (\ref{eq:OptimalAnythingProportions}), (\ref{eq:OptimalPackingProportions}) and (\ref{eq:OptimalMinimumProportions}), respectively. Select the exploration threshold equal to $f_\delta(t) =\log(C t^2/ \delta)$ with $C$ such that $C \geq e \sum_{t=1}^\infty (\frac{e}{K})^K\frac{(\log(Ct^2)\log(t))^K}{t^2}$. Then, \textsc{TaS} is $\delta$-PC, and its sample complexity satisfies on criteria $i$: for any $\boldsymbol{\mu}$ such that $k_\star$ is unique,
	\begin{equation}
		\limsup_{\delta \to 0} \frac{\mathbb{E}_{\boldsymbol{\mu}}[\tau]}{d_B(\delta,1-\delta)} \leq 2T_i(\boldsymbol{\mu}).
	\end{equation}
	\label{the:AlgResults}
\end{theorem}

We conclude this section by remarking that for $\boldsymbol{\mu}$ such that $k_\star$ is not unique, we would need to add a component to the algorithm to avoid the oscillation of $k_E(t)$ between these slices with minimal load. This is done in \cite{degenne2019pure} by introducing a {\it sticky} component to the algorithm. We could follow this idea, but for simplicity and clarity of the paper, prefer to restrict our attention to the cases where $k_\star$ is unique. 

==> Tech report version/Sections/B.UpperBoundProof.tex <==
\section{Upper bound proof and correctness of \textsc{TaS}}\label{appx:UpperBoundProofs}

In this section we prove Theorem \ref{the:AlgResults}. The proof logic closely follows that of \cite{garivier2016optimal}. We will show that this result is more generally applicable. 

First, take $\epsilon > 0$ and define the event $\mathcal{E}_T(\epsilon) = \bigcap_{t=\sqrt{T}}^T \{||\hat{\boldsymbol{\mu}}(t) - \boldsymbol{\mu}||_\infty < \xi(\epsilon)\}$, where $\xi(\epsilon)> 0$ is the greatest value such that 
%
\begin{align*}
||\boldsymbol{\mu}' - \boldsymbol{\mu}||_\infty < \xi(\epsilon) \implies &\mathcal{C}^\star(\boldsymbol{\mu}) \subseteq \mathcal{C}(\boldsymbol{\mu}'),\\
& ||\boldsymbol{w}^\star(\boldsymbol{\mu}') - \boldsymbol{w}^\star(\boldsymbol{\mu})||_\infty < \epsilon.
\end{align*}
%
Such $\xi(\epsilon)$ necessarily exists by continuity of $\boldsymbol{w}^\star$ (Proposition 6 of \cite{garivier2016optimal}, Theorem 4 of \cite{degenne2019pure}). Given a sufficiently small value of $\epsilon$, (say $\epsilon < \epsilon'(\boldsymbol{\mu})$ for some function $\epsilon'$) it holds that on $\mathcal{E}_T(\epsilon)$, $\hat{k}(t) \in \mathcal{C}^\star(\boldsymbol{\mu})$. We define $k_E(\boldsymbol{\mu}) = k_\star(\boldsymbol{\mu})$ in the case of packing-slice and $k_E(\boldsymbol{\mu}) = k^\star(\boldsymbol{\mu})$ in the case of any-available-slice or least-loaded-slice as the target of the true problem. On $\mathcal{E}_T(\epsilon)$ for $t \geq \sqrt{T}$, 
%
$$Q(t) = t \inf_{\boldsymbol{\lambda} \in \text{Alt}(k_E(\boldsymbol{\mu}))} D(\boldsymbol{n}(t)/t, \hat{\boldsymbol{\mu}}(t), \boldsymbol{\lambda}) .$$
%

Further, by Lemma 20 of \cite{garivier2016optimal}, for \textsc{TaS} there exists $T_\epsilon$ independent of $\delta$ such that for $T\geq T_\epsilon$ on $\mathcal{E}_T(\epsilon)$ it holds that $\forall t \geq \sqrt{T}$, $||\boldsymbol{n}(t)/t-\boldsymbol{w}^\star(\boldsymbol{\mu})||_\infty \leq 3(K-1)\epsilon$. Introducing $C^\star_\epsilon(\boldsymbol{\mu}) = \inf_{\boldsymbol{\mu}': ||\boldsymbol{\mu}' - \boldsymbol{\mu}||_\infty \leq \xi(\epsilon), \boldsymbol{w}': ||\boldsymbol{w}' - \boldsymbol{w}^\star(\boldsymbol{\mu})||_\infty \leq 3(K-1)\epsilon} D(\boldsymbol{w}', \boldsymbol{\mu}', \text{Alt}(\boldsymbol{\lambda}))$ it then follows that on $\mathcal{E}_T(\epsilon)$ for every $T \geq T_\epsilon$ and $t \geq \sqrt{T}$
%
$$
Q(t) \geq t C^\star_\epsilon(\boldsymbol{\mu}).
$$
%
Then, on $\mathcal{E}_T(\epsilon)$ and with $T \geq T_\epsilon$, we have
%
\begin{align*}
	\min(\tau_\delta, T) &\leq \sqrt{T} + \sum_{t=1}^T\mathds{1}_{(\tau_\delta > t)}
	\leq \sqrt{T} + \sum_{t=1}^T\mathds{1}_{(Q(t) \leq f_\delta(t))}\\
	&\leq \sqrt{T} + \sum_{t=1}^T\mathds{1}_{(tC^\star_\epsilon(\boldsymbol{\mu}) \leq f_\delta(T))}\leq \sqrt{T} +\frac{f_\delta(T)}{C^\star_\epsilon(\boldsymbol{\mu})} 
\end{align*}
%
Introducing $\tau_0(\delta) = \inf\{T: T\geq \sqrt{T} + \frac{f_\delta(T)}{C^\star_\epsilon(\boldsymbol{\mu})}\}$, it follows that for every $T\geq \max(\tau_0(\delta), T_\epsilon)$, $\mathcal{E}_T(\epsilon) \subseteq (\tau_\delta \leq T)$. As such, we have
%
\begin{align*}
	\E[\boldsymbol{\mu}]{\tau_\delta}&= \sum_{T=1}^\infty \mathbb{P}(\tau_\delta > T)\leq \tau_0(\delta) + T_\epsilon + \sum_{T=1}^\infty \mathbb{P}(\mathcal{E}_T^c(\epsilon))\\
	& \leq \tau_0(\delta) + T_\epsilon + \sum_{T=1}^\infty BT\exp(-CT^{1/8})
\end{align*}
%
where the final inequality follows from Lemma 19 in \cite{garivier2016optimal} for some constants $B$ and $C$ depending on $\epsilon$ and $\boldsymbol{\mu}$ but not $\delta$. Following the remainder of the proof step by step, we find that 
%
\begin{equation*}
	\limsup_{\delta \to 0} \frac{\E[\boldsymbol{\mu}]{\tau_\delta}}{\log(1/\delta)} \leq \limsup_{\delta \to 0} \frac{\tau_0(\delta)}{\log(1/\delta)} \leq \frac{2(1+\eta)}{C_\epsilon^\star(\boldsymbol{\mu})}
\end{equation*} 
for some $\eta > 0$ of our choice. By Theorem 4 of \cite{degenne2019pure}, the function $(\boldsymbol{w}, \boldsymbol{\mu})\mapsto D(\boldsymbol{w}, \boldsymbol{\mu}, \text{Alt}(\ell))$ is continuous on $\Lambda \times \mathcal{M}$ for any $\ell \in \mathcal{C}(\boldsymbol{\mu})$, so letting  $\epsilon \to 0$, $C^\star_\epsilon(\boldsymbol{\mu}) \to D(\boldsymbol{w}^\star(\boldsymbol{\mu}),\boldsymbol{\mu}, \text{Alt}(k_E(\boldsymbol{\mu})))$. But by Propositions \ref{prop:AnythingLowerBound}, \ref{prop:PackingLowerBound} and \ref{prop:MinimumLowerBound}, we see that this value is identical to $T_1(\boldsymbol{\mu})^{-1}$, $T_2(\boldsymbol{\mu})^{-1}$ and $T_3(\boldsymbol{\mu})^{-1}$ respectively, and we obtain the desired bound by letting $\eta \to 0$.

For the $\delta$-PC property, we will use a proof strategy similar to that of Proposition 12 in \cite{garivier2016optimal}. We will show that whenever an error occurs,  $f_\delta(t) < Q(t) < \sum_{k=1}^K n_k(t)(\hat{\mu}_k(t), \mu_k)$. Then, $\delta$-correctness follows from Theorem 2 in \cite{magureanu2014lipschitz}.

The first inequality is an immediate consequence of the statement of \textsc{TaS} (because errors occur only when the agent stops), so we focus on the second. For any-available-slice, packing-slice or least-loaded-slice, all errors can be divided into two categories, and we will show the inequality for both: 

(i) For some arm $\ell,\ \hat{\mu}_\ell(t) < \gamma < \mu_\ell$ or $\mu_\ell < \gamma < \hat{\mu}_\ell(t)$. In either case, for this to be considered an error it must be true that $Q(t) \leq n_\ell(t) d(\hat{\mu}_\ell(t), \gamma) < n_\ell(t) d(\hat{\mu}_\ell(t),\mu_\ell) \leq \sum_{k=1}^K n_k(t)d(\hat{\mu}_k(t),\mu_k)$, which concludes this category.

(ii) For some arms $j, \ell:$ $\hat{\mu}_j(t) < \hat{\mu}_\ell(t)$ and $\mu_\ell < \mu_j$. Defining $\alpha = n_j(t)/(n_j(t) + n_\ell(t))$, if this is considered an error, it can be shown (se the proof of Proposition 12 in \cite{garivier2016optimal}) that,  $Q(t) < n_j(t) d(\hat{\mu}_j(t), \alpha \hat{\mu}_j(t) + (1-\alpha)\hat{\mu}_\ell(t)) + n_\ell(t) d(\hat{\mu}_\ell(t), \alpha \hat{\mu}_j(t) + (1-\alpha)\hat{\mu}_\ell(t)) \leq n_j(t)d(\hat{\mu}_j(t),\mu_j) + n_\ell(t)d(\hat{\mu}_\ell(t),\mu_\ell) \leq \sum_{k=1}^K n_k(t)d(\hat{\mu}_k(t),\mu_k)$. This concludes the proof.


==> Tech report version/Sections/FutureWork.tex <==
Mean rewards of arms evolve as a stochastic process with 'memory'. 
$\Rightarrow$ Sequential best arm identification in non-stationary environments

